On the Mechanistic Interpretability of Neural Networks for Causality in Bio-statistics

Interpretable insights from predictive models remain critical in bio-statistics, particularly when assessing causality, where classical statistical and machine learning methods often provide inherent clarity. While Neural Networks (NNs) offer powerful capabilities for modeling complex biological data, their traditional "black-box" nature presents challenges for validation and trust in high-stakes health applications. Recent advances in Mechanistic Interpretability (MI) aim to decipher the internal computations learned by these networks. This work investigates the application of MI techniques to NNs within the context of causal inference for bio-statistics. We demonstrate that MI tools can be leveraged to: (1) probe and validate the internal representations learned by NNs, such as those estimating nuisance functions in frameworks like Targeted Minimum Loss-based Estimation (TMLE); (2) discover and visualize the distinct computational pathways employed by the network to process different types of inputs, potentially revealing how confounders and treatments are handled; and (3) provide methodologies for comparing the learned mechanisms and extracted insights across statistical, machine learning, and NN models, fostering a deeper understanding of their respective strengths and weaknesses for causal bio-statistical analysis.

==> Makefile <==
# partly autogenerated, that's why it's so ugly!

# say 'make V=1' to see the full build output
ifndef V
Q = @
Q_LATEX = sh -c 'echo -e "   " `echo $$(basename "$$0") | tr a-z A-Z`"\t$${!\#/..\/..\//}"; ! "$$0" "$$@" | grep -A5 -E "^[^ ]+:[0-9]+:"'
Q_OTHER = sh -c 'echo -e "   " `echo $$(basename "$$0") | tr a-z A-Z`"\t$${!\#/..\/..\//}"; "$$0" "$$@" >/dev/null'
endif

LATEX = latex
PDFLATEX = pdflatex
BIBTEX = bibtex
DVIPS = dvips
DVIPDF = dvipdf
PDFTOEPS = pdftops -eps
PDFTOPS = pdf2ps
EPSTOPDF = epstopdf
FIGTODEV = fig2dev
MPOST = mpost

.PHONY: all clean archive

all:  thesis

texfiles = $(wildcard *.tex)

.PHONY: thesis
thesis: thesis.pdf thesis.ps

thesis.pdf: $(texfiles) thesis.bbl
	$(Q) rm -rf build/pdf/; mkdir -p build/pdf/
	$(Q) cd build/pdf/ && TEXINPUTS="../../:$$TEXINPUTS" $(Q_LATEX) $(PDFLATEX) -interaction=nonstopmode -file-line-error ../../thesis.tex
	$(Q) cd build/pdf/ && TEXINPUTS="../../:$$TEXINPUTS" $(Q_LATEX) $(PDFLATEX) -interaction=nonstopmode -file-line-error ../../thesis.tex
	$(Q) ln -f build/pdf/thesis.pdf thesis.pdf

thesis.dvi: $(texfiles) thesis.bbl
	$(Q) rm -rf build/dvi/; mkdir -p build/dvi/
	$(Q) cd build/dvi/ && TEXINPUTS="../../:$$TEXINPUTS" $(Q_LATEX) $(LATEX) -interaction=nonstopmode -file-line-error ../../thesis.tex
	$(Q) cd build/dvi/ && TEXINPUTS="../../:$$TEXINPUTS" $(Q_LATEX) $(LATEX) -interaction=nonstopmode -file-line-error ../../thesis.tex
	$(Q) ln -f build/dvi/thesis.dvi thesis.dvi

thesis.ps: thesis.dvi
	$(Q)$(Q_OTHER) $(DVIPS) -q thesis

thesis.aux: $(texfiles)
	$(Q) $(Q_LATEX) $(LATEX) -interaction=nonstopmode -file-line-error thesis.tex

thesis.bbl: thesis.aux
	$(Q)$(Q_OTHER) $(BIBTEX) thesis

clean:
	rm -rf build/
	rm -f *.aux
	rm -f thesis.dvi thesis.idx thesis.ind thesis.ilg thesis.out thesis.toc thesis.pdf thesis.log

archive: thesis-template.zip

thesis-template.zip: *.tex Makefile ETHlogo.* refs.bib
	mkdir -p thesis
	cp `git ls-files "*.tex" Makefile "ETHlogo.*" refs.bib` thesis/
	perl -i -pe 's/\$$VERSION\$$/'"$$(git describe)/" thesis/*.tex
	rm -f thesis-template.zip
	zip -r thesis-template.zip thesis/


==> sections/Bonuses.tex <==
\chapter{Bonus: Other things I did during my thesis}

\section{HAL and implementing the algorithm in python}

\section{Investigating SAEs with Topological Data Analysis}

==> sections/_oldCausality.tex <==
\chapter{Causality, Bio-statistics, and the Targeted Learning Framework}
\label{chap:causality_tl}

\section{Fundamentals of Statistical Inference in Bio-statistics}
\label{sec:fundamentals_stats}

Before delving into advanced causal inference methodologies like Targeted Learning, it's essential to revisit fundamental concepts from statistical inference that form the bedrock of analyzing data from clinical trials and observational studies in bio-statistics. These concepts help us make decisions and draw conclusions about populations based on sample data, while explicitly acknowledging the inherent uncertainty.

\subsection{Hypothesis Testing}
\label{subsec:hypothesis_testing}
A fundamental part of traditional statistical analysis, particularly in clinical trials, is hypothesis testing. The primary goal is to evaluate the strength of evidence provided by the data against a specific claim or hypothesis about a population parameter, known as the \textit{null hypothesis} ($H_0$). Typically, $H_0$ represents a statement of "no effect" or "no difference." For example, in a drug trial, $H_0$ might state that the new drug has no effect on patient recovery time compared to a placebo.

Contrasting the null hypothesis is the \textit{alternative hypothesis} ($H_1$ or $H_a$), which represents what we aim to find evidence for – typically, the presence of an effect or difference (e.g., the drug \textit{does} improve recovery time).

The process involves calculating a test statistic from the sample data, which measures how far the observed data deviates from what would be expected under $H_0$. This leads to the computation of a \textit{p-value}. The p-value is the probability of observing a test statistic as extreme as, or more extreme than, the one actually observed, \textit{assuming the null hypothesis is true}.

Researchers typically set a pre-defined significance level, denoted by $\alpha$ (commonly 0.05), as a threshold for decision-making. If the p-value is less than or equal to $\alpha$, the result is deemed "statistically significant," and we reject $H_0$ in favor of $H_1$. If the p-value is greater than $\alpha$, we fail to reject $H_0$, meaning the data do not provide sufficient evidence against it at the chosen significance level.

\paragraph{Type I Error (False Positive)}Rejecting the null hypothesis ($H_0$) when it is actually true. The probability of making a Type I error is equal to the significance level $\alpha$. (e.g., concluding a drug is effective when it is not).
\paragraph{Type II Error (False Negative)}Failing to reject the null hypothesis ($H_0$) when it is actually false. The probability of making a Type II error is denoted by $\beta$. (e.g., failing to detect that a truly effective drug works).

\subsection{Statistical Power and Sample Size Considerations}
\label{subsec:stat_power}
Closely related to the Type II error is the concept of \textit{statistical power}, defined as $1 - \beta$. Power represents the probability that the test will correctly reject a false null hypothesis. In practical terms, it's the probability of detecting a true effect when one actually exists.

Adequate statistical power (often targeted at 80\% or higher) is crucial for the validity and efficiency of a study. An underpowered study (low power) has a high risk of failing to detect a real treatment effect, potentially leading to incorrect conclusions. Conversely, an overpowered study might use more resources (e.g., enroll more patients) than necessary.

Power is influenced by several factors:
\begin{itemize}
    \item \textbf{Effect Size:} The magnitude of the difference or effect being investigated. Larger effects are easier to detect, leading to higher power.
    \item \textbf{Sample Size (n):} The number of observations in the study. Larger sample sizes generally lead to higher power.
    \item \textbf{Significance Level ($\alpha$):} A higher $\alpha$ (e.g., 0.10 vs. 0.05) increases power but also increases the risk of a Type I error.
    \item \textbf{Data Variability:} Lower variability (e.g., smaller standard deviation) in the outcome measure increases power.
\end{itemize}
Power calculations are therefore essential during the study design phase to determine the minimum sample size required to have a reasonable chance of detecting a clinically meaningful effect, if it exists.

\subsection{Estimation and Confidence Intervals}
\label{subsec:estimation_ci}
While hypothesis testing primarily addresses the question of \textit{whether} an effect exists (statistical significance), \textit{estimation} focuses on quantifying the \textit{magnitude} of that effect. A \textit{point estimate} provides a single "best guess" for the value of a population parameter based on the sample data (e.g., the observed difference in mean recovery time between the drug and placebo groups).

However, a point estimate alone does not convey the uncertainty associated with it, which arises from sampling variability. To quantify this uncertainty, we compute a \textit{confidence interval (CI)}. A CI provides a range of plausible values for the true, unknown population parameter, calculated from the sample data.

% A common interpretation of a 95\% confidence interval is that if the study were repeated many times, and a 95\% CI was calculated from each study's sample, then approximately 95\% of those intervals would contain the true population parameter. It does \textit{not} mean there is a 95\% probability that the true value lies within the specific interval calculated from a single study.

Confidence intervals are often more informative than p-values alone because they provide information about both the magnitude of the effect (the point estimate) and its precision (the width of the interval). A narrow CI suggests a precise estimate, while a wide CI indicates considerable uncertainty. Examining whether a CI includes the value representing "no effect" (e.g., a difference of zero, or a ratio of one) can also be used for inference, often aligning with the conclusions from hypothesis testing.




\section{Causality in Bio-statistical Settings}
\label{sec:causality_biostats}

While fundamental statistical inference provides tools to describe data and test associations, a primary goal in many bio-statistical investigations, particularly in evaluating treatments or understanding disease etiology, is to determine \textit{causal} relationships. Does a specific drug \textit{cause} patient improvement? Does exposure to an environmental factor \textit{cause} an increase in disease risk? Answering such questions requires moving beyond mere association to establish causality, a significantly more challenging task.

\subsection{Defining Causal Effects}
\label{subsec:defining_causal_effects}
To formally discuss causality, statisticians often employ the \textit{Potential Outcomes Framework}, also known as the Neyman-Rubin Causal Model. Let's consider a simple scenario with a binary treatment (e.g., receiving a drug, denoted by $A=1$, versus receiving a placebo or standard care, $A=0$) and an outcome of interest (e.g., blood pressure level, denoted by $Y$).

For each individual $i$ in a population, we conceive of two \textit{potential outcomes}:
\begin{itemize}
    \item $Y_i(1)$: The outcome that \textit{would have been observed} if individual $i$ had received the treatment ($A=1$).
    \item $Y_i(0)$: The outcome that \textit{would have been observed} if individual $i$ had \textit{not} received the treatment ($A=0$).
\end{itemize}
The \textit{individual causal effect} for person $i$ is defined as the difference between their potential outcomes: $Y_i(1) - Y_i(0)$. This represents the true effect of the treatment specifically for that individual.

The fundamental challenge of causal inference is that we can only ever observe \textit{one} of the potential outcomes for any given individual. If the person received the treatment ($A=1$), we observe $Y_i = Y_i(1)$, but $Y_i(0)$ remains unobserved (counterfactual). If they did not receive the treatment ($A=0$), we observe $Y_i = Y_i(0)$, and $Y_i(1)$ is counterfactual.

Since individual causal effects are typically unobservable, we often focus on estimating \textit{average causal effects} at the population level. The most common target is the \textbf{Average Treatment Effect (ATE)}, defined as the expected difference in potential outcomes across the entire population:
\[ \text{ATE} = E[Y(1) - Y(0)] = E[Y(1)] - E[Y(0)] \]
The ATE represents the average impact we would expect to see if, hypothetically, everyone in the population received the treatment compared to if everyone received the control. Other causal parameters of interest might include the Average Treatment effect on the Treated (ATT), conditional causal effects within subgroups, or effects of time-varying treatments. This framework provides a precise mathematical language for defining the causal question we aim to answer.

\subsection{The Challenge of Causal Inference from Data}
\label{subsec:association_vs_causation}
A central tenet of statistics is that \textbf{association is not causation}. Observing that two variables, $A$ and $Y$, tend to vary together (i.e., they are associated or correlated) does not, by itself, imply that $A$ causes $Y$. For example, observing that patients taking a particular vitamin supplement ($A$) have lower rates of a certain illness ($Y$) does not automatically mean the supplement prevents the illness. It might be that healthier, more health-conscious individuals are more likely to take supplements \textbf{and} are independently less likely to become ill.

In a well-conducted \textit{Randomized Controlled Trial (RCT)}, the random assignment of treatment ($A$) ensures that, on average, the treatment group ($A=1$) and control group ($A=0$) are comparable in terms of all pre-treatment characteristics (both measured and unmeasured). Randomization breaks any systematic link between patient characteristics and the treatment they receive. Therefore, any observed difference in the average outcome between the groups, $E[Y|A=1] - E[Y|A=0]$, can be attributed to the causal effect of the treatment, providing a direct estimate of the ATE (under certain assumptions like no loss-to-follow-up).

However, RCTs are not always feasible, ethical, or practical. Much bio-statistical data comes from \textit{observational studies}, where individuals' exposures or treatments are not randomly assigned but occur for various reasons (patient choice, doctor's decision, environmental factors, etc.). In such studies, the groups being compared (e.g., treated vs. untreated) often differ systematically in ways related to the outcome, making the naive comparison $E[Y|A=1] - E[Y|A=0]$ a biased estimate of the causal effect $E[Y(1)] - E[Y(0)]$. Disentangling causation from association in observational data requires careful consideration of potential biases (see Appendix \ref{app:ACEBiased} for proof).

\subsection{Key Obstacles: Confounding and Bias}
\label{subsec:confounding_bias}
Several factors can obscure the true causal relationship between an exposure/treatment and an outcome in observational studies, and sometimes even in imperfect RCTs.

\paragraph{Confounding}This is perhaps the most critical challenge. A confounder is a variable that is associated with both the treatment/exposure ($A$) and the outcome ($Y$), independently of the exposure. It creates a spurious association (or masks a true one) between $A$ and $Y$. For example, in studying the effect of alcohol consumption ($A$) on mortality ($Y$), socioeconomic status ($C$) could be a confounder if people with lower socioeconomic status tend to drink more heavily \textbf{and} also have higher mortality rates due to other factors (like access to healthcare). Failing to account for confounders leads to \textit{confounding bias}.

\paragraph{Selection Bias}This occurs when the selection of individuals into the study, or into the analysis, is related to both the exposure and the outcome. This leads to the study sample being unrepresentative of the target population in a way that distorts the exposure-outcome relationship. Examples include:
\subparagraph{Differential loss-to-follow-up} If patients with worse outcomes are more likely to drop out of the treatment group than the control group.
\subparagraph{Healthy worker effect} Comparing mortality rates in an occupational cohort to the general population; workers are often healthier than the general population, biasing comparisons \citep{HealthyWorkerEffect}.
\subparagraph{Collider stratification bias} Conditioning on a variable that is a common effect of the exposure and the outcome (or factors related to them) can induce spurious associations.

Addressing these challenges requires careful study design and sophisticated analytical methods that go beyond simple comparisons.

\subsection{Introduction to Structural Causal Models (SCMs)}
\label{ssec:intro_scms_dags}
To formalize causal assumptions and guide analysis, researchers increasingly use \textit{Structural Causal Models (SCMs)}. An SCM represents hypothesized causal relationships among a set of variables. Often, these relationships are visualized using \textit{Directed Acyclic Graphs (DAGs)}.

In a DAG, \textbf{Nodes} represent variables (e.g., treatment $A$, outcome $Y$, confounders $C$) and \textbf{Directed Arrows (Edges)} represent direct causal effects. An arrow from $A$ to $Y$ ($A \rightarrow Y$) indicates the assumption that $A$ has a direct causal influence on $Y$ (relative to the other variables in the graph). The \textbf{Acyclicity} comes from the fact that no variable causes itself, directly or indirectly.

% DAGs provide a powerful visual language for:
% \begin{itemize}
%     \item \textbf{Explicitly stating causal assumptions:} Drawing a DAG forces clarity about the hypothesized data-generating process.
%     \item \textbf{Identifying confounders:} Using graphical criteria (like the "backdoor criterion"), DAGs help identify the set(s) of variables that must be measured and adjusted for in the analysis to remove confounding bias and isolate the causal effect of interest (e.g., the path $A \rightarrow Y$).
%     \item \textbf{Visualizing potential biases:} DAGs can illustrate how confounding paths or selection mechanisms might bias an analysis.
% \end{itemize}
% While the potential outcomes framework defines *what* causal effect we want to estimate, SCMs and DAGs provide a framework for representing the assumed causal structure of the world and identifying *how* we might estimate that effect from data, particularly by highlighting the necessary adjustments for confounding. Understanding these structures is fundamental to applying advanced causal inference methods, including Targeted Learning.

\section{The Targeted Learning Framework}
\label{sec:tl_framework}

The challenges inherent in estimating causal effects from observational data, primarily confounding and various forms of bias (as discussed in Section~\ref{sec:causality_biostats}), necessitate statistical methodologies that move beyond simple association measures or traditional regression techniques. Standard parametric models (e.g., linear or logistic regression) often rely on strong, potentially incorrect assumptions about the relationships between variables, leading to biased causal effect estimates if these assumptions are violated. Conversely, while modern machine learning (ML) offers powerful tools for flexible prediction, these algorithms are typically optimized for predictive accuracy rather than for estimating a specific causal parameter, and often lack straightforward procedures for constructing valid confidence intervals or assessing statistical significance for the causal effect.

\subsection{Motivation: Need for Robust and Efficient Causal Estimation}
\label{subsec:tl_motivation}
There is a critical need for a framework that can:
\begin{enumerate}
    \item \textbf{Formally define the causal question} as a specific parameter (the target parameter) of the underlying data-generating distribution, often grounded in the potential outcomes framework (Section~\ref{subsec:defining_causal_effects}).
    \item \textbf{Minimize reliance on restrictive parametric assumptions}, allowing for complex, non-linear relationships between variables as often occur in biological systems.
    \item \textbf{Leverage the predictive power of machine learning} to flexibly model parts of the data-generating process, such as the relationship between confounders and the outcome, or between confounders and the treatment assignment.
    \item \textbf{Provide valid statistical inference} for the target causal parameter, including asymptotically unbiased estimates, valid confidence intervals, and hypothesis tests.
    \item \textbf{Offer robustness}, ideally providing some protection against potential misspecification in the modeling process.
    \item \textbf{Achieve statistical efficiency}, making the best possible use of the available data to obtain precise estimates (i.e., narrow confidence intervals).
\end{enumerate}
The Targeted Learning (TL) framework, pioneered by Mark van der Laan and colleagues, was developed precisely to address these needs, offering a principled approach to integrate machine learning with causal inference methodology.

\subsection{The Targeted Learning Roadmap}
\label{subsec:tl_roadmap}
TL provides a general template, or roadmap, for constructing estimators of target parameters, particularly causal effects. It typically involves a two-stage process:

\paragraph{Stage 1: Initial Estimation of Nuisance Parameters}
The first step involves obtaining estimates of certain features of the data-generating distribution that are necessary for estimating the target parameter but are not of direct scientific interest themselves. These are often called \textit{nuisance parameters}. In causal inference, common nuisance parameters include:
\begin{itemize}
    \item The conditional expectation of the outcome given treatment and confounders, $E[Y|A, W]$ (the outcome regression).
    \item The conditional probability of receiving treatment given confounders, $P(A=1|W)$ (the treatment mechanism or propensity score).
\end{itemize}
Crucially, TL encourages the use of flexible, data-adaptive machine learning algorithms for this initial estimation step. Often, an ensemble method called \textbf{Super Learner} \citep{van2007super} is employed. Super Learner uses cross-validation to combine predictions from a diverse library of candidate ML algorithms (e.g., regression models, splines, random forests, gradient boosting, neural networks), selecting the best-performing combination based on theoretical results that guarantee asymptotically optimal prediction performance under certain conditions. This minimizes the risk of relying on a single, potentially misspecified model for these crucial nuisance components.

\paragraph{Stage 2: Targeting the Initial Estimates}
This is the key innovation of TL. The initial estimates from Stage 1, even if obtained using excellent ML algorithms, are optimized for overall prediction, not specifically for minimizing the bias of the final target parameter estimate. The targeting step adjusts, or "fluctuates," the initial estimate of the outcome regression (or sometimes other parts of the distribution) in a specific, minimal way. This adjustment is carefully constructed, typically using information from the estimated treatment mechanism (propensity score), to ensure that the updated estimate solves a particular statistical equation (the "efficient influence curve equation") related to the target parameter.

The primary goal of this targeting step is to reduce bias in the final estimate of the target parameter while minimally increasing variance. By solving the efficient influence curve equation, the resulting estimator gains desirable statistical properties, namely \textit{double robustness} and potential for \textit{asymptotic efficiency} (discussed further in Section~\ref{sec:tmle_estimator}). The final estimate of the target parameter is then calculated as a function of these targeted nuisance parameter estimates.

\subsection{Key Principles: Defining the Target Parameter and Using the Statistical Model}
\label{subsec:tl_principles}
Two foundational principles underpin the TL framework:

\paragraph{1. Clearly Define the Target Parameter:} Before any estimation begins, the scientific question must be translated into a precisely defined quantity, or \textit{parameter}, of the underlying probability distribution of the data. This parameter represents the causal effect or other feature of interest (e.g., the ATE, $E[Y(1)]-E[Y(0)]$). This clear definition is essential because the entire TL procedure, particularly the targeting step, is tailored to optimizing the estimation of this specific parameter. Without a well-defined target, the process lacks direction.

\paragraph{2. Operate within a Statistical Model:} TL operates within a defined \textit{statistical model}, which represents the set of possible probability distributions that could have generated the observed data. This model codifies our assumptions about the data. TL strongly advocates for using realistic, large statistical models, often \textit{non-parametric} or \textit{semi-parametric}, which make fewer assumptions than traditional parametric models. SCMs and DAGs (Section~\ref{subsec:intro_scms_dags}) are often used to help define the statistical model and the assumptions (like which variables are confounders) needed to identify the target causal parameter within that model. The goal of TL is then to produce an efficient and robust estimator of the target parameter within this chosen statistical model, leveraging data as much as possible while respecting the stated assumptions.

By combining a clear definition of the target parameter, the flexibility of machine learning within a potentially large statistical model, and a specific targeting step focused on the parameter of interest, TL provides a powerful and rigorous framework for causal inference in complex bio-statistical settings. Targeted Maximum Likelihood Estimation (TMLE) is the most prominent implementation of this framework.

\section{Targeted Maximum Likelihood Estimation (TMLE)}
\label{sec:tmle_estimator}

Targeted Maximum Likelihood Estimation (TMLE) stands as the most prominent and widely used estimation strategy developed within the TL framework \citep{vanderLaanRubin2006}. It provides a concrete, general algorithm for implementing the TL roadmap described in Section~\ref{subsec:tl_roadmap}, yielding estimators that possess desirable statistical properties like double robustness and asymptotic efficiency, making them particularly suitable for causal inference in complex bio-statistical settings.

\subsection{Conceptual Overview of the TMLE Algorithm}
\label{subsec:tmle_algorithm}
The TMLE algorithm follows the two-stage structure of the TL roadmap. For estimating a target parameter like the Average Treatment Effect (ATE = $E[Y(1)] - E[Y(0)]$), the typical steps are:

\paragraph{1. Initial Estimation of Nuisance Parameters:}
First, obtain initial estimates for the relevant nuisance parameters using the observed data $(W_i, A_i, Y_i)$ for $i=1, ..., n$, where $W$ represents the set of baseline confounders. These typically include:
\begin{itemize}
    \item $\bar{Q}^0(A, W)$: An initial estimate of the conditional mean of the outcome given treatment and confounders, $E[Y|A, W]$. This is often obtained using Super Learner (Section~\ref{subsec:tl_roadmap}) to fit $Y$ on $A$ and $W$.
    \item $g^0(W)$: An initial estimate of the treatment mechanism (propensity score), $P(A=1|W)$. This is also frequently estimated using Super Learner to fit the binary treatment indicator $A$ on $W$.
\end{itemize}
These initial estimates aim for good predictive performance based on the observed data.

\paragraph{2. Targeting Step (Fluctuation):}
This crucial step adjusts the initial outcome regression estimate $\bar{Q}^0(A, W)$ to make it more focused on optimizing the bias for the specific target parameter (e.g., the ATE). This is achieved by:
\begin{itemize}
    \item Defining a "clever covariate" (also known as the "updating covariate" or part of the "efficient influence curve") that depends on the treatment $A$ and the estimated propensity score $g^0(W)$. For the ATE, a common form of this covariate is $H(A,W) = \left( \frac{I(A=1)}{g^0(W)} - \frac{I(A=0)}{1-g^0(W)} \right)$, where $I(\cdot)$ is the indicator function. This covariate essentially incorporates information about the treatment assignment mechanism into the outcome regression update.
    \item Fitting a simple parametric regression model (often a logistic regression for binary $Y$ or a linear regression for continuous $Y$) for the outcome $Y$, using the initial prediction $\bar{Q}^0(A, W)$ as an offset (or on the scale of the linear predictor for logistic regression) and the clever covariate $H(A,W)$ as the sole predictor. This model typically takes the form: $Y \sim \text{offset}(\bar{Q}^0(A, W)) + \epsilon H(A,W)$.
    \item Estimating the coefficient $\epsilon$ of the clever covariate using Maximum Likelihood Estimation (MLE) based on the observed data. This fitting step gives TMLE its name.
    \item Updating the initial estimate $\bar{Q}^0(A, W)$ using the fitted $\epsilon$ and the clever covariate to obtain the targeted estimate $\bar{Q}^*(A, W)$. For example, if using logistic regression, the update might look like $\text{logit}(\bar{Q}^*(A, W)) = \text{logit}(\bar{Q}^0(A, W)) + \hat{\epsilon} H(A,W)$.
\end{itemize}
This fluctuation step ensures that the resulting targeted estimate $\bar{Q}^*(A, W)$ satisfies a key statistical property related to the efficient influence curve of the target parameter, which is essential for achieving double robustness and efficiency.

\paragraph{3. Final Parameter Estimation:}
Once the targeted estimate $\bar{Q}^*(A, W)$ is obtained, the final estimate of the target parameter is computed. For the ATE, this involves:
\begin{itemize}
    \item Predicting the potential outcomes under treatment ($A=1$) and control ($A=0$) for each individual using the targeted estimate: $\bar{Q}^*(1, W_i)$ and $\bar{Q}^*(0, W_i)$.
    \item Averaging these predicted potential outcomes across all individuals in the sample.
    \item Calculating the difference: $\hat{\psi}_{\text{TMLE}} = \frac{1}{n} \sum_{i=1}^{n} [\bar{Q}^*(1, W_i) - \bar{Q}^*(0, W_i)]$.
\end{itemize}
This final value $\hat{\psi}_{\text{TMLE}}$ is the TMLE estimate of the ATE.

\paragraph{4. Statistical Inference:}
Confidence intervals and p-values for the TMLE estimate are typically derived using the estimate of its \textit{influence curve (IC)}. The IC characterizes the asymptotic behavior of the estimator. An estimate of the IC can be calculated for each observation using the targeted nuisance parameter estimates ($\bar{Q}^*$ and $g^0$). The variance of the TMLE estimate is then estimated as the sample variance of the estimated IC values, divided by the sample size $n$. Standard Wald-type confidence intervals and hypothesis tests can then be constructed.

\subsection{Key Properties of TMLE}
\label{subsec:tmle_properties}
The carefully constructed targeting step endows TMLE with two highly desirable statistical properties.

\paragraph{Double Robustness}
The TMLE estimator for the target parameter (e.g., ATE) is \textit{doubly robust} (or \textit{doubly protected}). This means that the estimator $\hat{\psi}_{\text{TMLE}}$ will be consistent (i.e., it converges to the true value $\psi_0$ as the sample size $n \to \infty$) if \textit{either} the initial outcome regression $E[Y|A,W]$ is estimated consistently \textit{or} the propensity score $P(A=1|W)$ is estimated consistently. It is not necessary for \textit{both} initial nuisance parameter estimates to be correct.
\subparagraph{Advantage} This provides significant protection against model misspecification. In practice, correctly modeling both complex relationships ($Y$ on $A,W$ and $A$ on $W$) can be difficult. Double robustness increases the chance of obtaining a valid causal estimate even if one of the models is misspecified. Using Super Learner for both nuisance parameters further enhances this practical advantage, as it increases the likelihood that at least one of the estimates will perform well.

\paragraph{Asymptotic Efficiency}
If \textit{both} the outcome regression $E[Y|A,W]$ and the propensity score $P(A=1|W)$ are estimated consistently (and at appropriate convergence rates, often achievable with Super Learner), then the TMLE is typically \textit{asymptotically efficient} within the class of regular, asymptotically linear estimators for the chosen statistical model.
\subparagraph{Advantage} This means that, under ideal conditions (both nuisance models correctly specified), TMLE achieves the lowest possible asymptotic variance. It extracts the maximum amount of information from the data regarding the target parameter, leading to the most precise estimates and the narrowest possible confidence intervals among well-behaved estimators.

In summary, TMLE provides a systematic approach to estimating causal parameters (and other complex parameters) by leveraging machine learning for flexibility (via initial estimation, often with Super Learner) and incorporating a targeted update step rooted in statistical theory. This targeting step ensures the resulting estimator is not only data-adaptive but also doubly robust and potentially achieves optimal statistical efficiency, making TMLE a powerful tool for rigorous causal inference in bio-statistics.


\section{Extensions and Applications of TMLE}
\label{sec:tmle_extensions}

The flexibility and robust theoretical underpinnings of Targeted Maximum Likelihood Estimation have led to its adaptation and extension for a wide range of complex scenarios encountered in bio-statistics and beyond. The core principles of defining a target parameter, obtaining initial nuisance parameter estimates, and performing a targeted update remain central, but the specific implementation details evolve to address different data structures and scientific questions.

\subsection{Longitudinal TMLE (LTMLE)}
\label{subsec:ltmle}
Many bio-statistical studies involve longitudinal data, where individuals are followed over time, and treatments, exposures, confounders, and outcomes are measured repeatedly. Estimating the causal effect of a time-varying treatment strategy (e.g., initiating medication based on evolving patient status) presents significant challenges not present in the static (single time point) setting.

A key difficulty is \textit{time-varying confounding affected by past treatment}. This occurs when a variable measured at a specific time point acts as a confounder for the treatment-outcome relationship at a later time point, but this variable's value is itself influenced by earlier treatment decisions. For example, in studying the long-term effect of an anti-inflammatory drug, a patient's measured inflammation level at month 6 might influence the decision to continue the drug at month 7 (acting as a confounder) but might also have been affected by whether the patient received the drug between months 0 and 6 (affected by past treatment). Standard methods like conventional regression or simple propensity score matching fail in the presence of such feedback loops.

\textit{Longitudinal TMLE (LTMLE)} \citep{vanderLaanRobins2003, bang_robins_2005, vanderLaanPetersenHubbard2008} extends the TMLE framework specifically to handle these complexities. It typically involves:
\begin{itemize}
    \item Defining a causal parameter relevant to the longitudinal setting (e.g., the effect of a sustained treatment strategy versus no treatment on the final outcome).
    \item Sequentially estimating the required nuisance parameters (outcome regressions and treatment probabilities) backward or forward in time, appropriately conditioning on the observed past history at each time point. This often involves fitting a series of models, one for each time interval.
    \item Performing a sequential targeting step, often iterating backward from the final time point, to ensure the final estimator satisfies the appropriate longitudinal efficient influence curve equation.
\end{itemize}
LTMLE provides a doubly robust and potentially efficient method for estimating causal effects of dynamic treatment regimes and time-varying exposures from longitudinal observational data, properly accounting for time-varying confounding.

\subsection{Deep TMLE: Integrating Machine Learning Advances}
\label{subsec:deep_tmle}
As machine learning continues to advance, particularly in the realm of deep learning (using artificial neural networks with multiple layers), there is growing interest in integrating these powerful predictive models within the TMLE framework. \textit{Deep TMLE} refers to implementations where NNs are used, sometimes within a Super Learner ensemble, for the initial estimation of the nuisance parameters ($E[Y|A, W]$ and/or $P(A=1|W)$).

The motivation stems from the ability of NNs to automatically learn complex, high-dimensional, and non-linear patterns directly from data, potentially improving the accuracy of the initial nuisance parameter estimates, especially when dealing with:
\begin{itemize}
    \item High-dimensional covariate data ($W$).
    \item Complex interactions between variables.
    \item Data with inherent structures like images or sequences (e.g., time series in longitudinal data).
\end{itemize}
By potentially providing better initial estimates, DNNs might help TMLE get closer to achieving its theoretical efficiency gains in practice. The core targeting step of TMLE remains unchanged; it simply operates on the initial estimates provided by the DNN (or a Super Learner including DNNs).

However, using DNNs within TMLE also introduces considerations regarding computational cost, hyperparameter tuning complexity for the networks, and the "black-box" nature of some deep learning models, although the overall double robustness property of TMLE still applies based on the consistency of the nuisance function estimates, regardless of the specific algorithm used.

\subsubsection{Example: DragonNet -- Adapting Neural Networks for the Estimation of Treatment Effects \citep{shi2019adapting}}\label{subsubsec:deep_ltmle_dragonnet_example}

\subsubsection{Example: LTMLE with TD Heterogeneous Transformer \citep{shirakawa_deepltmle_2024}}
\label{subsubsec:deep_ltmle_transformer_example}
A cutting-edge application combining these ideas is presented in \citep{shirakawa_deepltmle_2024}, which explores using advanced deep learning architectures within the LTMLE framework for longitudinal data. Specifically, this work likely leverages the Transformer architecture (cf. section \ref{ssec:transformers}) to model the complex temporal dependencies inherent in longitudinal nuisance functions (e.g., how the outcome at time $t$ depends on the entire history of past treatments and covariates).
The Transformer's "attention mechanism" is particularly adept at capturing long-range dependencies and interactions over time, potentially offering advantages over simpler recurrent neural networks or standard regression models when modeling $E[Y_t | \bar{A}_{t-1}, \bar{W}_{t-1}]$ or $P(A_t=1 | \bar{A}_{t-1}, \bar{W}_t)$ (where $\bar{X}_t$ denotes the history of variable $X$ up to time $t$). The "TD Heterogeneous" aspect likely refers to handling time-dependent (TD) data with potentially varying types of variables (heterogeneous).

By embedding such a sophisticated sequence model within the LTMLE algorithm for nuisance parameter estimation, followed by the standard LTMLE targeting step, this approach aims to harness the predictive power of state-of-the-art deep learning while retaining the causal inference rigor (double robustness, efficiency guarantees) provided by the TL framework. This exemplifies how TMLE can be integrated with ongoing ML advancements to tackle increasingly complex causal questions in dynamic settings.

\subsection{Other TMLE Variants}
\label{subsec:other_tmle}
The TMLE framework has been further adapted for various other statistical tasks, demonstrating its versatility:
\begin{itemize}
    \item \textbf{Conditional Average Treatment Effects (C-TMLE):} Estimates the average treatment effect within specific subgroups defined by baseline covariates ($E[Y(1)-Y(0)|V]$ where $V \subset W$). This is useful for understanding treatment effect heterogeneity.
    \item \textbf{Mediation Analysis TMLE:} Estimates direct and indirect causal effects, seeking to understand the mechanisms through which a treatment influences an outcome (e.g., how much of a drug's effect on mortality is mediated through its effect on blood pressure).
    \item \textbf{TMLE for Optimal Dynamic Treatment Regimes:} Used to estimate the optimal sequence of treatments tailored to individual patient characteristics evolving over time.
    \item \textbf{TMLE for Survival Analysis:} Adapts TMLE for time-to-event outcomes, handling censoring appropriately while estimating causal effects on survival probabilities or restricted mean survival times.
\end{itemize}
These extensions highlight TMLE as a general methodology applicable whenever the goal is robust and efficient estimation of a specific target parameter within a given statistical model.


\section{Comparison with Other Causal Inference Methods}
\label{sec:comparison_methods}

Targeted Maximum Likelihood Estimation (TMLE) represents a sophisticated approach to causal inference, but it exists alongside several other established methods designed to estimate causal effects, particularly from observational data. Understanding the conceptual differences and theoretical properties of these methods helps appreciate the specific advantages offered by the TL framework. Here, we briefly contrast TMLE with Inverse Probability Weighting (IPW), Standardization (G-computation), and Propensity Score Matching (PSM).

\subsection{Inverse Probability Weighting (IPW):}
\begin{itemize}
    \item \textbf{Mechanism:} IPW aims to create a pseudo-population where the treatment assignment ($A$) is independent of the measured confounders ($W$). It achieves this by weighting each individual $i$ by the inverse of the probability of receiving the treatment they actually received, conditional on their confounders ($1/P(A=A_i|W=W_i)$). This probability is the propensity score ($g(W)$ for $A=1$) or $1-g(W)$ (for $A=0$). The causal effect is then estimated using a simple weighted comparison of outcomes between treatment groups in this pseudo-population.
    \item \textbf{Modeling Focus:} Primarily relies on correctly modeling the treatment mechanism (propensity score), $P(A|W)$. The outcome model $E[Y|A, W]$ is not directly used in the standard IPW estimator.
    \item \textbf{Robustness:} IPW is generally \textit{singly robust}. Its consistency depends crucially on the correct specification of the propensity score model. If the PS model is wrong, the IPW estimate will typically be biased.
    \item \textbf{Efficiency \& Challenges:} IPW can be inefficient, especially if some individuals have very low probabilities of receiving the treatment they got (leading to extreme weights). This instability can inflate variance and make the estimator sensitive to outliers or model misspecification in the tails of the propensity score distribution. Stabilized weights are often used to mitigate this but don't eliminate the core reliance on the PS model.
    \item \textbf{Contrast with TMLE:} Unlike IPW's sole reliance on $P(A|W)$, TMLE utilizes estimates of *both* $P(A|W)$ and $E[Y|A, W]$ and combines them in a way (via the targeting step) that achieves double robustness. TMLE does not involve explicit weighting of individuals, avoiding the extreme weight instability issue.
\end{itemize}

\subsection{Standardization / G-computation:}
\begin{itemize}
    \item \textbf{Mechanism:} Standardization, often referred to as G-computation in the context of causal inference \citep{Robins1986}, directly estimates the outcome regression model $E[Y|A, W]$. It then uses this model to predict the potential outcome for every individual under treatment ($A=1$) and under control ($A=0$), using their observed covariates $W$. The average potential outcomes $E[Y(1)]$ and $E[Y(0)]$ are estimated by averaging these predictions over the entire sample distribution of $W$. The ATE is the difference between these averages.
    \item \textbf{Modeling Focus:} Primarily relies on correctly modeling the outcome regression, $E[Y|A, W]$. The propensity score is not directly used for estimation (though it can be useful for diagnostics).
    \item \textbf{Robustness:} Standardization is also generally \textit{singly robust}. Its consistency depends crucially on the correct specification of the outcome model. If the outcome model is wrong (e.g., misses important interactions or non-linearities), the estimate will typically be biased.
    \item \textbf{Efficiency \& Challenges:} Its efficiency depends on the accuracy of the outcome model. It can be challenging to correctly specify this model, especially with many confounders or complex relationships.
    \item \textbf{Contrast with TMLE:} TMLE also estimates $E[Y|A, W]$ but includes the crucial targeting step, which incorporates information from the propensity score estimate $P(A|W)$ to improve robustness and efficiency. Standard G-computation lacks this targeting step and the resulting double robustness property.
\end{itemize}

\subsection{Propensity Score Matching (PSM):}
\begin{itemize}
    \item \textbf{Mechanism:} PSM first estimates the propensity score $P(A|W)$ for each individual. It then attempts to match treated individuals ($A=1$) with one or more control individuals ($A=0$) who have very similar propensity scores. The idea is that within matched sets, the distribution of observed confounders $W$ should be similar between treated and control units, mimicking randomization. The treatment effect is estimated by comparing outcomes within these matched pairs or sets.
    \item \textbf{Modeling Focus:} Primarily relies on correctly modeling the propensity score, $P(A|W)$. The outcome model is not directly used.
    \item \textbf{Robustness:} Like IPW, PSM is generally \textit{singly robust}, depending on the correct specification of the propensity score model.
    \item \textbf{Efficiency \& Challenges:} PSM often discards unmatched individuals, potentially reducing sample size and efficiency. Finding good matches can be difficult, especially in high dimensions or when the propensity score distributions have poor overlap (violating the positivity assumption). It is difficult to adapt for continuous treatments, and deriving appropriate standard errors can be complex.
    \item \textbf{Contrast with TMLE:} TMLE uses the entire sample and doesn't rely on finding explicit matches. It uses the propensity score in a different way (within the targeting step or via Super Learner) rather than for matching. TMLE generally offers a more direct path to estimating standard errors and tends to be more efficient as it uses all data points.
\end{itemize}

% \subsection{other stuff from the different papers like DeepACE or whatever \citep{DeepACE}}


%\textbf{Summary of TMLE Advantages:}
%Compared to these traditional methods, TMLE (within the broader TL framework) offers significant theoretical advantages:
%\begin{itemize}
%    \item \textbf{Double Robustness:} Provides protection against misspecification of *either* the outcome model *or* the propensity score model, unlike singly robust methods (IPW, G-computation, PSM).
%    \item \textbf{Potential for Efficiency:} Aims to achieve the lowest possible asymptotic variance when both nuisance models are correctly specified.
%    \item \textbf{Systematic Framework:} Provides a clear roadmap that readily incorporates modern machine learning (via Super Learner) for flexible nuisance parameter estimation while retaining valid statistical inference.
%    \item \textbf{Direct Estimation:} Directly targets the parameter of interest, often leading to more stable estimation than methods relying on %weighting or exact matching.
%\end{itemize}
%While practical performance can depend on the specific dataset, sample size, and quality of model fitting, TMLE's strong theoretical properties make it an attractive and increasingly preferred method for causal inference, especially in complex bio-statistical applications where model misspecification is a significant concern.  

==> sections/_oldMechanisticinterpretability.tex <==
\chapter{Mechanistic Interpretability as a proxy learning tool for bio-statistic modeling}\label{chap:mech_int}

Mechanistic Interpretability (MI) aims to unravel the internal workings of machine learning models, particularly complex NNs, to understand \textit{how} they arrive at decisions rather than just assessing \textit{what} decisions they make. This endeavor moves beyond treating models as "black boxes" towards achieving a deeper, causal understanding of their computations. In the context of bio-statistics, especially for high-stakes applications like survival prediction, such understanding is not merely academically interesting but critical for ensuring model reliability, transparency, safety, and ethical deployment. As models grow in complexity (cf. Figure 1.1), trading predictive capability for interpretability, MI offers a suite of techniques to potentially regain understanding without sacrificing performance.

% This chapter explores several key MI techniques, drawing from recent advancements in the field. It examines how these methods can be conceptualized and potentially applied as proxy learning tools within bio-statistical modeling frameworks, such as the Targeted Learning (TL) approach discussed in Chapter \ref{chap:causality_tl}. We will discuss activations as the fundamental units of information, methods to interpret them like probing and patching, techniques like Sparse Autoencoders (SAEs) for feature disentanglement, Causal Abstraction for model validation, the role of synthetic data, and finally, how these tools collectively serve as proxies for understanding complex bio-statistical models.

This chapter explores multiple MI techniques, drawing from most recent advancements in the field. While most techniques are developed around natural language and reasoning tasks, we conceptualized and leveraged them as proxy learning tools within bio-statistical modeling frameworks. 

\section{Techniques of Mechanistic Interpretability}
\label{sec:techniques_of_mi}
%Activations are the numerical outputs of neurons (or nodes) within a neural network after an activation function has been applied (cf. Section \ref{sec:neuron_act}). They represent the flow and transformation of information through the network's layers, from the initial input representation to the final prediction layer. Understanding activations is fundamental to MI, as they provide a window into the model's internal state and learned representations at various stages of computation. Analyzing these activations allows researchers to hypothesize about the concepts, features, or patterns the model utilizes internally.
Activations (cf. Section \ref{ssec:neuron_act}) are the backbone of MI techniques. They indeed reveal the true computations happening within the NN, allowing to delve into complex computations. Most of the time, those computations are even too difficult to comprehend, as modern NN deal with very abstract concepts flowing through billions and billions of parameters.

\subsection{Probing}
\label{subsec:probing}
Probing refers to a set of techniques used to investigate the information encoded within a model's activations. Typically, this involves training a simple, auxiliary classifier (the "probe") on the activations extracted from intermediate layers of a pre-trained NN to predict specific properties or concepts \citep{alain2017understanding}. The performance of the probe is then used as evidence for whether the chosen layer's activations encode the target property.

In bio-statistics, probing could be employed to determine if specific layers of a survival prediction model encode relevant biological markers, patient demographic information, disease stage indicators, or treatment history features. For instance, one might train a probe on the activations of a model processing patient electronic health records (EHR) to see if it can predict the presence of a specific comorbidity.

However, research suggests that probing primarily reveals observational correlations – what information is \textit{present} in the activations – rather than demonstrating that the model causally \textit{uses} that information for its final prediction \citep{Belinkov2022ProbingClassifiers}. A successful probe indicates encoding, but not necessarily functional relevance. Thus, probing results are often best interpreted in conjunction with interventional methods. An analogy can be drawn from studies on game-playing AI like AlphaZero, where probing revealed the encoding of strategic chess concepts \citep{McGrath2022}; similarly, probing in biostats might reveal encoded risk factors, but further analysis is needed to confirm their influence on the survival prediction.

% \subsection{Activation Patching/Ablation}
% \label{subsec:activation_patching}
% Activation patching and ablation are causal intervention techniques designed to go beyond the observational nature of probing and determine the functional role of specific activations or neuron groups within a model's computation \citep{vig2020causal, Meng2022LocatingAE}.

\subsection{Activation Patching} typically involves running the model on two different inputs: a "clean" input and a "corrupted" or contrasting input. During the forward pass on the clean input, the activations at a specific layer or location are "patched" – replaced with the corresponding activations generated from the corrupted input. The effect of this substitution on the model's final output (e.g., the predicted survival probability) is then measured. A significant change in output suggests the patched activations play a causal role in processing the features that differ between the clean and corrupted inputs \citep{wang2022interpretability}.

Add another thing about what can be measured, how does it relate to causal settings (having submodel? already CA, donc parler de juste les rapports de cusalité intra model et du savoir qu'on peu en tirer, en mode causal scrubbing

\subsection{Ablation} is a simpler intervention where specific activations (e.g., corresponding to a neuron or a channel) are set to a neutral value, often zero, effectively removing their contribution. Observing the impact on model performance or output helps determine the necessity of that component.

In bio-statistics, activation patching could be used to verify if specific internal features learned by a survival model, perhaps hypothesized to represent tumor characteristics, are indeed causally influential in predicting patient outcomes. By patching activations between runs with data from patients with different tumor types, one could isolate the model components responsible for differentiating between them. Ablation could identify critical neurons whose removal significantly degrades prediction accuracy.

Extensions like path patching (analyzing specific computation pathways) and tools like Patchscopes \citep{ghandeharioun2024patchscopes} provide more fine-grained analysis. However, challenges remain, such as designing meaningful clean/corrupted input pairs or templates and accounting for potential compensatory effects or "second-order effects" where the network adapts to the intervention in complex ways. These interventions are crucial for ensuring that models used in medical predictions rely on genuinely relevant features rather than spurious correlations, aligning model behavior with established medical knowledge.

\subsection{Causal Tracing}

\subsection{Circuit Analysis}

\subsection{Sparse AutoEncoder \& Transcoders}
\label{sec:sae_transcoders}
While activations provide raw data about internal states, interpreting them directly can be difficult, especially due to phenomena like polysemanticity, where a single neuron activates in response to multiple unrelated concepts \citep{Elhage2022ToyMO}. Sparse Autoencoders (SAEs) and, to a lesser extent currently, Transcoders, are techniques aimed at decomposing complex activation patterns into more interpretable, potentially monosemantic features.

\textbf{Sparse Autoencoders (SAEs)} are unsupervised models trained to reconstruct the activations of a specific layer in a larger, pre-trained NN (cf. Section \ref{sec:autoencoders}). An SAE typically consists of an encoder that maps the original activations to a higher-dimensional, but sparsely activated, latent space, and a decoder that reconstructs the original activations from this sparse representation \citep{cunningham2023sparse}. The sparsity constraint encourages the SAE to learn an "overcomplete basis" where individual dimensions (features) in the sparse latent space correspond to distinct, interpretable concepts or directions within the original activation space.

% In bio-statistics, SAEs could be applied to the internal layers of a complex survival prediction model (perhaps a deep NN or Transformer trained on multimodal data). The learned sparse features might correspond to specific clinical indicators, genetic markers, image textures, or combinations thereof that influence the survival prediction. Identifying these features could provide novel biological insights or confirm that the model leverages known prognostic factors. Research has shown SAEs scaling to large language models \citep{cunningham2023sparse, kissane2024finding} and identifying safety-relevant features, suggesting potential for complex bio-statistical models.

\textbf{Transcoders} are a less established technique but share the goal of enhancing interpretability through sparsity. They aim to approximate a dense layer or block within a network using a sparser, more interpretable structure. For example, sparse distillation techniques might train a transcoder layer that mimics the function of a dense layer while using fewer active pathways or features \citep{dunefsky2024transcoders}. This simplification could make the model's internal computations more transparent. For biostats models, a transcoder might simplify a complex feature extraction layer, revealing a sparser set of core factors driving predictions. However, research on transcoders is nascent, and challenges include robust evaluation methods, especially without ground-truth knowledge of the underlying features.

\subsection{Causal Abstraction}
\label{sec:causal_abstraction}
Causal abstraction provides a formal framework for analyzing and validating the causal structure of computations within NNs \citep{Geiger2021CausalAO}. It treats parts of a neural network (from individual neurons to entire layers or modules) as nodes in a causal graph and uses interventions to verify hypothesized causal relationships between these components and the model's output or behaviour. The core idea is to abstract the detailed computations into higher-level causal variables and relationships that are easier to understand and reason about.

A key technique within this framework is the use of \textit{interchange interventions} \citep{Geiger2021CausalAO}. Similar in spirit to activation patching, these interventions involve swapping internal states (activations) between model runs on different inputs that vary along specific, hypothesized causal dimensions. If the model's output changes predictably according to the hypothesized causal relationship after the swap, it provides evidence for the validity of the abstraction.

Causal abstraction aims to unify various interpretability methods, including causal mediation analysis and correlational approaches like probing, under a single causal lens. Recent work has focused on scaling these methods, for instance, using techniques like distributed alignment search to find corresponding causal variables across different models or layers \citep{Geiger2023Distributed}.

% For bio-statistical modeling, causal abstraction offers a rigorous way to validate whether a survival prediction model's reasoning aligns with domain knowledge. For example, if we hypothesize that a specific module in the network processes information about treatment effectiveness, causal abstraction could test this by intervening on the module's activations and observing if the output changes in a way consistent with known treatment effects. This verification is crucial for building trust and ensuring the ethical use of predictive models in healthcare, confirming that predictions rely on causally sound mechanisms rather than just correlational patterns. It helps bridge the gap between the model's internal computations and the causal understanding expected in medical science.

\section{Proxy Learning Tools}
\section{Merging Ideas of Mechanistic interpretability and Bio-statistics}
\subsection{Sampling Synthetic Data}
\label{sec:synthetic_data}
While not always categorized as a standalone MI technique, the use of synthetic data plays a crucial role in understanding and validating NN behaviour in controlled settings. Synthetic datasets can be generated with known properties, ground-truth causal relationships, or specific statistical distributions, allowing researchers to test hypotheses about model learning dynamics and internal representations.

Several MI-related approaches implicitly or explicitly leverage synthetic data:
\begin{itemize}
    \item \textbf{Feature Visualization:} Techniques aiming to understand what individual neurons or channels represent often involve generating synthetic inputs (e.g., via optimization) that maximally activate that component \citep{olah2017feature, Zeiler2014}.
    \item \textbf{Toy Models and Phenomena Study:} Researchers often use simple, synthetic datasets to study fundamental NN phenomena like superposition \citep{Elhage2022ToyMO}, grokking \citep{Power2022Grokking}, or phase transitions in learning, isolating these behaviours in a controlled environment.
    \item \textbf{Controlled Benchmarking:} Synthetic data allows for the creation of benchmarks where the presence and influence of specific features (e.g., confounders, mediators) are known a priori, enabling rigorous testing of whether a model correctly identifies and utilizes causal structures.
\end{itemize}

In bio-statistics, particularly for survival analysis, generating synthetic patient data can be invaluable. One could simulate EHR data based on known biological processes, disease progression models, or treatment effect mechanisms. By training a survival prediction model on this synthetic data, researchers can assess:
\begin{itemize}
    \item Whether the model correctly captures the known underlying hazard rates or survival distributions.
    \item If the model identifies the pre-defined prognostic factors and correctly estimates their influence.
    \item How the model behaves in the presence of known confounders or time-varying covariates, testing the effectiveness of frameworks like LTMLE (cf. Section \ref{subsec:ltmle}) when combined with NNs.
    \item Using MI techniques (like probing or patching) on models trained on synthetic data where the ground truth is known can help validate the interpretability methods themselves.
\end{itemize}
By verifying model behaviour and interpretations against synthetic data with known ground truths, we can build confidence before applying these models and MI techniques to complex, noisy real-world patient data where the underlying causal mechanisms are often uncertain.

\section{Proxy learning on survival prediction}
\label{sec:proxy_learning}
The concept of "proxy learning" in this context refers to the use of MI techniques as tools to approximate, understand, and potentially even guide the learning process of complex bio-statistical models, particularly for survival prediction. Given the often high dimensionality of bio-statistical data (e.g., genomics, imaging, EHRs) and the complexity of modern predictive models (e.g., deep learning architectures), direct interpretation or validation can be intractable. MI techniques can serve as "proxies" for understanding by focusing on specific aspects of the model's internal mechanisms.

We can synthesize the application of the previously discussed MI techniques as components of this proxy learning approach for survival prediction:
\begin{itemize}
    \item \textbf{Probing as a proxy for feature representation:} Use probing to check if the model internally represents known clinical risk factors or biological markers relevant to survival, serving as a proxy for verifying that the model has learned relevant domain knowledge.
    \item \textbf{Activation Patching as a proxy for causal relevance:} Employ patching interventions to test the causal impact of specific internal model components (e.g., neurons encoding a treatment response feature) on the final survival prediction. This acts as a proxy for understanding the functional role of different parts of the model.
    \item \textbf{SAEs as a proxy for disentangled factors:} Apply SAEs to decompose complex internal activations into sparse, interpretable features. These features (e.g., representing specific comorbidities or genetic expressions) serve as proxies for the underlying factors driving the model's prediction.
    \item \textbf{Causal Abstraction as a proxy for mechanistic alignment:} Use causal abstraction to validate if the high-level causal structure inferred from the model aligns with established medical pathways or biological understanding, acting as a proxy for overall model trustworthiness.
    \item \textbf{Synthetic Data as a proxy for controlled validation:} Leverage synthetic survival data with known properties to test if the model and the MI-derived interpretations hold up in controlled scenarios, serving as a proxy for expected real-world generalization.
\end{itemize}

By employing this suite of MI techniques as proxies, we can gain valuable insights into complex survival models that might otherwise remain opaque. This proxy understanding is crucial for:
\begin{itemize}
    \item \textbf{Transparency and Trust:} Making the model's decision-making process clearer to clinicians, researchers, and regulators.
    \item \textbf{Ethical Considerations:} Ensuring predictions are based on medically relevant factors and not biased by spurious correlations related to sensitive attributes.
    \item \textbf{Model Debugging and Improvement:} Identifying internal flaws or unexpected behaviour (e.g., reliance on artifacts) that could be rectified.
    \item \textbf{Scientific Discovery:} Potentially uncovering novel biomarkers or interactions learned by the model from data.
\end{itemize}

While challenges remain regarding the scalability, fidelity, and completeness of MI techniques \citep{cunningham2023sparse}, using them collectively as proxy learning tools offers a promising pathway to bridge the gap between the predictive power of complex models and the need for understanding and reliability in bio-statistical applications like survival prediction. This chapter has outlined how these techniques, from analyzing activations to validating causal abstractions, contribute to this goal, setting the stage for empirical investigation within the TL framework.


% McGrath2022 (AlphaZero chess knowledge):

% Likely Reference: McGrath, T., Gregg, J., Nix, A., Pedregosa, F., Hechtman, B., Kramár, J., ... & Hassabis, D. (2022). Acquisition of Chess Knowledge in AlphaZero. Proceedings of the National Academy of Sciences (PNAS), 119(20), e2117210119.

% Context: This paper explicitly analyzes how AlphaZero learns concepts like king safety, piece value, etc., aligning with the description.

% alain2017understanding (Probing basics):

% Likely Reference: Alain, G., & Bengio, Y. (2017). Understanding Intermediate Layers Using Linear Classifier Probes. International Conference on Learning Representations (ICLR). (arXiv preprint arXiv:1610.01644, 2016).

% Context: This is a foundational paper on using linear probes to understand representations in neural networks.

% Belinkov2022ProbingClassifiers (Probing limitations/observational nature):

% Likely Reference: Belinkov, Y. (2022). Probing Classifiers: Promises, Pitfalls, and Best Practices. Transactions of the Association for Computational Linguistics (TACL), 10, 1141-1159. (arXiv preprint arXiv:2108.08326, 2021).

% Context: This paper provides a critical review of probing methods, discussing their limitations, including the correlation vs. causation issue mentioned.

% vig2020causal (Activation patching/causal methods - mediation):

% Likely Reference: Vig, J., Gehrmann, S., Belinkov, Y., Qian, S., Nevo, D., Singer, Y., & Shieber, S. (2020). Investigating Gender Bias in Language Models Using Causal Mediation Analysis. Advances in Neural Information Processing Systems (NeurIPS), 33, 12388-12401.

% Context: While focused on bias, this paper applies causal mediation analysis, a related concept to intervention-based methods like patching, to understand model internals. Note: Direct "activation patching" might also trace to other works, but Vig et al. is prominent in causal analysis of LMs.

% Meng2022LocatingAE (Activation patching/causal methods - locating/editing):

% Likely Reference: Meng, K., Bau, D., Andonian, A., & Belinkov, Y. (2022). Locating and Editing Factual Associations in GPT. Advances in Neural Information Processing Systems (NeurIPS), 35, 17359-17372. (Often referred to as ROME - Rank-One Model Editing).

% Context: This work uses causal tracing (related to patching) to locate where factual information is stored and methods to edit it, fitting the description.

% wang2022interpretability (Activation patching details/causal role):

% Likely Reference: Wang, K., Variengien, A., …, & Steinhardt, J. (2022). Interpretability in the Wild: A Circuit for Indirect Object Identification in GPT-2 small. arXiv preprint arXiv:2211.00593.

% Context: This is a well-known paper demonstrating circuit analysis in GPT-2 using techniques including activation patching to determine the causal roles of components.

% ghandeharioun2024patchscopes (Patchscopes):

% Likely Reference: Ghandeharioun, A., et al. (2024). Patchscopes: A Unifying Framework for Inspecting Hidden Representations of Language Models. International Conference on Learning Representations (ICLR).

% Context: Directly matches the name and concept.

% Elhage2022ToyMO (Polysemanticity/Superposition):

% Likely Reference: Elhage, N., et al. (2022). Toy Models of Superposition. Anthropic. (Available online: https://transformer-circuits.pub/2022/toy_model/index.html).

% Context: This is the primary work from Anthropic discussing the concept of superposition (related to polysemanticity) using toy models.

% cunningham2023sparse (Sparse Autoencoders - scaling/safety):

% Likely Reference: Cunningham, H., et al. (2023). Sparse Autoencoders Find Highly Interpretable Features in Language Models. arXiv preprint arXiv:2309.08600. (While dated 2023, it's the seminal work discussed widely into 2024 regarding scaling and finding features, including safety-relevant ones).

% Alternative/Related: Bricken, T., et al. (2023). Towards Monosemanticity: Decomposing Language Models With Dictionary Learning. arXiv preprint arXiv:2310.15911. (Builds on SAEs).

% Context: This line of work from Anthropic focuses specifically on using SAEs to find interpretable features in large models, fitting the description. The text's mention of "(2024)" might refer to its ongoing impact or later updates/blog posts.

% kissane2024finding (SAEs in transformers):

% Uncertain Reference: The summary text might be slightly misattributing or referring to very recent/unpublished work. A related paper is: Kissane, A., et al. (2024). Finding Neurons in a Haystack: Case Studies with Sparse Probing. International Conference on Learning Representations (ICLR). However, this uses sparse probing, not SAEs directly for feature decomposition as implied by the context alongside Cunningham.

% Action: It might be best to cite Cunningham et al. (2023) or Bricken et al. (2023) for SAE applications in transformers and either omit Kissane or clarify its distinct approach (sparse probing) if relevant. Double-check the source of the summary text if possible.

% dunefsky2024transcoders (Transcoders/Sparse Distillation):

% Likely Reference: Dunefsky, E., et al. (2024). Learning Sparse Transcoders for Neural Network Interpretability. International Conference on Learning Representations (ICLR).

% Context: Directly matches the name and concept.

% Geiger2021CausalAO (Causal Abstraction framework/interchange interventions):

% Likely Reference: Geiger, A., et al. (2021). Causal Abstractions of Neural Networks. Advances in Neural Information Processing Systems (NeurIPS), 34, 24247-24258.

% Context: This is the foundational paper introducing the formal framework of causal abstraction and interchange interventions for NNs.

% Geiger2023Distributed (Causal Abstraction scaling/distributed alignment search):

% Likely Reference: Geiger, A., et al. (2023). Finding Alignments Between Interpretable Causal Variables. International Conference on Machine Learning (ICML).

% Context: This paper addresses scaling causal abstraction by finding alignments between variables, matching the description of distributed alignment search.

% olah2017feature (Feature visualization):

% Likely Reference: Olah, C., Mordvintsev, A., & Schubert, L. (2017). Feature Visualization. Distill. doi:10.23915/distill.00007

% Context: A seminal article on methods for visualizing what features neurons learn.

% Power2022Grokking (Grokking phenomenon):

% Likely Reference: Power, A., et al. (2022). Grokking: Generalization Beyond Overfitting on Small Algorithmic Datasets. arXiv preprint arXiv:2201.02177.

% Context: The paper that introduced and studied the "grokking" phenomenon in NNs.



==> sections/_oldMechanisticinterpretability2.tex <==
\chapter{Mechanistic Interpretability for Analyzing Neural Networks in Causal Bio-statistical Settings}\label{chap:mech_int}

\section{Goals of Mechanistic Interpretability in this Context}
* Briefly define MI (understanding internal mechanisms, moving beyond input-output).
* Specific Aims for Bio-statistics \& TL:
* Validation: Verify if NN components (e.g., used for nuisance functions in TMLE) learn representations consistent with domain knowledge (e.g., known risk factors, confounders).
* Discovery: Uncover potentially novel biological/causal relationships or patient subgroups learned by the NN.
* Debugging \& Robustness: Identify reliance on spurious correlations or artifacts vs. genuine causal features.
* Comparison: Understand how NN mechanisms differ from or align with traditional statistical models used in causal inference.
* Trustworthiness: Build confidence in NN predictions by understanding why they are made.



\section{Core Techniques of Mechanistic Interpretability}\label{sec:techniques_of_mi}

\subsection{Observational Techniques: What Information is Encoded?}\label{ssec:observational_techniques}
Observational techniques aim to understand the information represented within a neural network's internal states -- activations -- without altering the network's computation during inference. The core question these methods address is: \textit{Given a specific input, what kind of information is encoded in the activation patterns at different layers of the network?} These techniques passively observe the network's function to map its internal representations to human-understandable concepts. One of the most common observational methods is probing.

\subsubsection{Probing}
\textbf{Probing}, often referred to as linear probing, is a technique used to determine if specific properties or concepts are encoded in a neural network's intermediate representations. The fundamental idea is to train a \textit{simple} (often linear) supervised model, the \textbf{probe}, on the activation vectors extracted from a specific layer of a pre-trained network to predict a target property associated with the original input.

Let $f$ be a pre-trained neural network. We are interested in understanding the representations at a specific layer $l$. For a dataset of inputs $\{x_i\}$, we first compute the corresponding activation vectors $\{h^{(l)}_i\}$ at layer $l$ by performing a forward pass: $h^{(l)}_i = f^{(l)}(x_i)$, where $f^{(l)}$ denotes the computation up to layer $l$.
Alongside the inputs $\{x_i\}$, we have corresponding labels $\{y_i\}$ representing the property we want to probe for (e.g., a biological marker, a demographic attribute, a linguistic feature). These labels $y_i$ are \textit{not} necessarily the original labels used to train the main network $f$.

We then train a separate, simple classifier $g$ (the probe) that takes the activations $h^{(l)}_i$ as input and attempts to predict the property labels $y_i$:
$$ \hat{y}_i = g(h^{(l)}_i) $$
The probe $g$ is deliberately kept simple (e.g., logistic regression, a linear Support Vector Machine (SVM), or a shallow (MLP)) for a crucial reason. The goal is not to achieve the absolute best possible prediction accuracy for $y_i$, but rather to assess how \textit{easily} (e.g., linearly) the information about $y_i$ can be extracted from the activations $h^{(l)}_i$. If a simple probe $g$ achieves high performance (measured on a held-out test set using metrics like accuracy, F1-score, etc.) in predicting $y_i$ from $h^{(l)}_i$, it suggests that the information related to the property $y$ is explicitly represented or readily available in the activations at layer $l$. Conversely, poor performance suggests the information is either absent, obfuscated, or encoded in a highly non-linear way that the simple probe cannot capture.

\paragraph{Correlation, not Causation}
A critical limitation of probing, inherent to its observational nature, is that it can only reveal \textbf{correlation}, not \textbf{causation}. A successful probe demonstrates that information about property $y$ is \textit{present} in the activations $h^{(l)}$, meaning the activations correlate with $y$. However, it \textit{does not} prove that the main network $f$ actually \textit{uses} this information causally to arrive at its final prediction. The network might encode the information incidentally, perhaps because the probed property $y$ is correlated with other features the network \textit{does} use. As highlighted by works like \citep{ProbingClassifiers2022}, interpreting probe results requires caution; high accuracy indicates representation, but not necessarily utilization. To assess causal reliance, interventional techniques (discussed in Section~\ref{sec:interventional_techniques}) are necessary.


\subsection{Interventional Techniques: What Mechanisms Does the Model Causally Rely On?}\label{ssec:interventional_techniques}

While observational techniques like probing (Section~\ref{ssec:observational_techniques}) reveal correlations between neural network activations and specific concepts, they cannot establish \textit{causal} links. They tell us what information is \textit{present}, but not necessarily what information the model \textit{uses} to make its predictions. \textbf{Interventional techniques} address this gap by actively manipulating the network's internal state during computation and observing the effect on the output. By changing specific activations or component functions, we can test hypotheses about whether those components causally contribute to the model's behavior.

\subsubsection{Activation Patching / Interchange Interventions}
\textbf{Activation Patching} and \textbf{Interchange Interventions} are powerful interventional techniques designed to isolate the causal effect of specific internal activations on the model's output.

The core idea is to perform \textbf{swapping activations between runs on different inputs}. It involves running the model on two inputs:
\begin{enumerate}
    \item A \textbf{base input} ($x_{base}$), representing the default or clean state for which we want to understand the computation.
    \item A \textbf{source input} ($x_{source}$), representing a state containing a specific feature or condition whose effect we want to isolate.
\end{enumerate}
The model is run forward on both inputs. At a specific, pre-determined point in the network (e.g., the output of a specific neuron, a set of neurons, an attention head output, or an entire layer activation vector $h^{(l)}$), the activation value computed during the forward pass on the base input ($h^{(l)}_{base}$) is discarded. Instead, the corresponding activation value computed from the source input ($h^{(l)}_{source}$) is "patched" into the computation for the base input. The forward pass for the base input then resumes from this point using the patched activation $h^{(l)}_{source}$.

Mathematically, if $f$ is the network and $f_{>l}$ denotes the computation from layer $l+1$ onwards, the original output for the base input is $y_{base} = f(x_{base}) = f_{>l}(f^{(l)}(x_{base}))$. The patched output is $y_{patched} = f_{>l}(h^{(l)}_{source})$. The difference between $y_{patched}$ and $y_{base}$ measures the causal effect of the information encoded in the activation at layer $l$ specifically related to the difference between $x_{source}$ and $x_{base}$, on the final output for $x_{base}$.


\subsubsection{Ablation}
\textbf{Ablation} is a conceptually simpler, yet fundamental, interventional technique. It involves \textbf{zeroing/neutralizing components} of the neural network to understand their contribution. This typically means setting the output of specific components (e.g., individual neurons, attention heads, residual stream components, or even entire layers) to zero during the forward pass. Essentially, the component is "removed" from the computation for that specific run. 

The primary goal of ablation is to identify \textbf{critical neurons/layers} or other components necessary for the model's performance or a specific behavior. By observing the degradation in performance (e.g., drop in accuracy, increase in loss) or the change in output when a component is ablated, we can infer its importance. If ablating a neuron significantly harms performance on a task, that neuron is considered \textit{causally important} for that task. 

Ablation is often a \textit{first step} in understanding model mechanisms due to its simplicity. While less nuanced than activation patching (which replaces information rather than just removing it), ablation effectively answers the question: "\textit{Is this component necessary for the observed behavior?}"


\subsubsection{Causal Tracing}
\textbf{Causal Tracing} is an interventional technique, often built upon activation patching, that aims to \textbf{trace the flow of effects from interventions} through the network's layers. While a single activation patch measures the effect of a source activation at a specific layer $l$ on the final output, causal tracing extends this to understand how that effect propagates through intermediate layers.

The core idea is to investigate not just the final output change, but also how activations at intermediate layers $k > l$ are affected when an activation at layer $l$ is patched from a source input $x_{source}$ into the computation of a base input $x_{base}$. Specifically, one might perform an activation patch at layer $l$ (replacing $h^{(l)}_{base}$ with $h^{(l)}_{source}$) and then measure the change in activations at a subsequent layer $k$: $\Delta h^{(k)} = h^{(k)}_{patched} - h^{(k)}_{base}$. A significant change $\Delta h^{(k)}$ suggests that the causal pathway from the information difference introduced at layer $l$ passes through layer $k$.

Causal tracing helps pinpoint \textit{where} an effect originating earlier in the network (represented by the patched activation) has its impact on later representations, and \textit{how} different components (e.g., specific neurons or attention heads in subsequent layers) respond to the patched information, revealing the computational pathway.


\subsubsection{Causal Scrubbing}
\textbf{Causal Scrubbing} provides a methodology to evaluate whether a hypothesized computational structure, represented as an abstraction of the neural network $f$, is sufficient to explain a target behavior, often measured via a loss function $L$.

This evaluation begins by formalizing the hypothesis. This typically involves defining a \textbf{high-level interpretation graph}, $G_{HL} = (V_{HL}, E_{HL})$, which captures the hypothesized critical computational components $V_{HL}$ and their causal dependencies $E_{HL}$. This graph is often conceptualized as a SCM (cf. Section~\ref{ssec:intro_scms_dags}). A \textbf{translation function}, $\tau: V_{HL} \rightarrow \mathcal{P}(V_{LL})$, maps these high-level nodes to their corresponding elements (sets of neurons, attention heads, etc.) $V_{LL}$ within the actual network's computational graph (the \textbf{low-level graph}).

The methodology then proceeds by performing targeted interventions on the network's internal activations during a forward pass for a given input $x_{base}$. Specifically, it uses \textbf{behavior-preserving resampling ablations}. For certain nodes $v \in V_{LL}$ in the low-level graph, their original activation $h_v(x_{base})$ is replaced (``scrubbed'') with an activation $h'_v$. This replacement activation $h'_v$ is typically generated by running the network on a different input, $x_{resample}$, i.e., $h'_v = h_v(x_{resample})$. Critically, the choice of which nodes $v$ to scrub and how to select $x_{resample}$ is constrained by the dependencies specified in the high-level hypothesis graph $G_{HL}$. If a node $v$ is part of a high-level component $u \in V_{HL}$ (i.e., $v \in \tau(u)$), its resampling might depend on ensuring consistency with the parents of $u$ in $G_{HL}$, $Pa_{HL}(u)$. Nodes $v$ corresponding to high-level components hypothesized to be irrelevant, or nodes considered conditionally independent based on $G_{HL}$'s structure, can be resampled more freely (e.g., using a randomly chosen $x_{resample}$ or one matching only necessary parent conditions). Let $f_{scrubbed}(x_{base})$ denote the output of the network after performing all specified scrubbing interventions based on $G_{HL}$.

The validity of the hypothesis $G_{HL}$ is then quantitatively assessed by measuring how well the model's original behavior is preserved under these interventions, typically evaluated over a dataset $D$. This is often quantified by comparing the expected loss after scrubbing, $\mathbb{E}_{x \sim D}[L(f_{scrubbed}(x))]$, to the original expected loss, $\mathbb{E}_{x \sim D}[L(f(x))]$. If the loss remains largely unchanged, meaning the difference $\Delta L = \mathbb{E}_{x \sim D}[L(f_{scrubbed}(x))] - \mathbb{E}_{x \sim D}[L(f(x))]$ is close to zero (high recovery), it provides strong evidence that the hypothesized structure $G_{HL}$ accurately captures the necessary mechanisms for the behavior. This is because altering parts of the network outside this hypothesized structure (or altering parts within it according to the hypothesized conditional independencies) did not significantly disrupt performance. Conversely, a significant increase in loss ($\Delta L \gg 0$, low recovery) indicates the hypothesis $G_{HL}$ is incomplete or incorrect, as the scrubbing interventions disrupted computations essential to the behavior that were not accounted for in the hypothesis.

\subsection{Feature Analysis and Decomposition: What Concepts Are Represented?}
Beyond understanding causal reliance through interventions, another crucial aspect of MI is analyzing the features or concepts represented within a network's activations. Techniques in this category aim to decompose complex, often high-dimensional activation vectors into more understandable or meaningful components.

\subsubsection{Sparse Autoencoders}
\textbf{Sparse Autoencoders (SAEs)} are an unsupervised machine learning technique specifically adapted to analyze internal network activations. They are structured as AEs (cf Section~\ref{sec:autoencoders}), comprising an encoder function $f_{enc}$ and a decoder function $f_{dec}$, trained not on the original input data, but on the activation vectors $h^{(l)}$ extracted from an intermediate layer $l$ of a pre-trained base model $f$. The primary objective is to \textbf{reconstruct these activations sparsely}. That is, the SAE learns a mapping such that $h^{(l)} \approx f_{dec}(f_{enc}(h^{(l)}))$, but with a crucial constraint imposed on the latent representation $z = f_{enc}(h^{(l)})$: the vector $z$ must be sparse, meaning most of its components are zero for any given activation $h^{(l)}$.

The core goal of employing SAEs is to find potentially \textbf{monosemantic features} within the network's representations, thereby helping to overcome the common issue of \textbf{polysemanticity}. Polysemanticity occurs when individual neurons or units in the base model $f$ respond to multiple, seemingly unrelated concepts or features in the input data. An SAE attempts to address this by decomposing the potentially polysemantic activation vector $h^{(l)} \in \mathbb{R}^d$ into a typically higher-dimensional latent code $z \in \mathbb{R}^k$ (where $k \gg d$) that is constrained to be sparse. The hypothesis is that this sparsity encourages each non-zero component $z_j$ of the latent code (often called a "feature activation") to correspond to a single, more interpretable underlying concept or property represented within $h^{(l)}$.

The standard SAE approach trains the encoder and decoder parameters ($\theta_{enc}, \theta_{dec}$) to minimize a loss function balancing reconstruction accuracy with sparsity. A common formulation uses L1 regularization:
$$ L_{SAE}(\theta_{enc}, \theta_{dec}) = \mathbb{E}_{h^{(l)}} \left[ ||h^{(l)} - f_{dec}(f_{enc}(h^{(l)}))||^2_2 + \lambda ||f_{enc}(h^{(l)})||_1 \right] $$
Here, the first term is the reconstruction loss (e.g., MSE), and the second term penalizes the L1 norm of the latent code $z = f_{enc}(h^{(l)})$, weighted by $\lambda$, encouraging sparsity. However, several distinct variants of SAEs have emerged. An alternative method is the \textbf{TopK sparse autoencoder}, which directly controls sparsity by keeping only the $k$ largest activations in $z$ and zeroing out the rest. This approach can simplify hyperparameter tuning compared to tuning $\lambda$ and potentially achieve a better trade-off on the reconstruction-sparsity frontier. The choice of activation function itself significantly impacts feature stability; for instance, \textbf{ReLU-based SAEs} have shown greater consistency in learned features across different random initializations compared to some state-of-the-art TopK variants \citep{Paulo2025}. Other strong alternatives include \textbf{JumpReLU} SAEs \citep{Rajamanoharan2024} employing the following specific activation function within the encoder:
$$\text{JumpReLU}_\theta(z) \coloneqq z H(z-\theta)$$
where $H$ is the  Heaviside step function (cf. Section~\ref{ssec:mlp}) and $\theta>0$ is the JumpReLU’s threshold.

\subsubsection{Transcoders}
\textbf{Transcoders} are another mechanistic interpretability technique aiming for \textbf{sparse and interpretable mappings}, but specifically designed to analyze neural network \textbf{computation flows across consecutive layers}, particularly within FFN sublayers. Unlike Sparse Autoencoders which typically decompose activation vectors $h^{(l)}$ at a single layer $l$, transcoders focus on approximating the transformation performed by a network component mapping from the pre-component activations to the post-component activations. Structurally, a transcoder utilizes an encoder $f_{enc}$ and a decoder $f_{dec}$ to mimic the function $f_{FFN}$ of a target FFN layer, often using an overparameterized, wider latent space $z = f_{enc}(h^{(l)})$ that is constrained to be sparse.

The primary objective is to \textbf{decompose complex neural computations into interpretable circuits}. This addresses the challenge that neurons in standard FFNs often activate densely, making direct circuit analysis difficult. By enforcing sparsity in the latent space that represents the transformation itself, transcoders encourage the discovery of factorized computational pathways, potentially separating input-dependent and input-invariant aspects of the layer's function and yielding more interpretable circuits.

Transcoders are trained to minimize a loss function that balances the fidelity of approximating the FFN's transformation with the sparsity of the intermediate latent representation $z$. This loss typically takes the form:
$$ L_{transcoder}(\theta_{enc}, \theta_{dec}) = \mathbb{E}_{h^{(l)}} \left[ ||f_{FFN}(h^{(l)}) - f_{dec}(f_{enc}(h^{(l)}))||^2_2 + \lambda_1 ||f_{enc}(h^{(l)})||_1 \right] $$
Here, $h^{(l)}$ represents the input activation to the target FFN layer, $f_{FFN}(h^{(l)})$ is the true output activation of that layer, and the first term measures the reconstruction error between the true output and the transcoder's approximation. The second term is an L1 sparsity penalty on the latent code $z = f_{enc}(h^{(l)})$, controlled by the hyperparameter $\lambda_1$.

By focusing on the transformation $h^{(l)} \rightarrow f_{MLP}(h^{(l)})$ rather than just the representation $h^{(l)}$, transcoders enable a different kind of analysis compared to SAEs. They facilitate weights-based circuit analysis \textit{through} a layer, offering insights into how information is processed and transformed, potentially providing a more robust way to elicit and reverse-engineer latent computational circuits within larger models.


\subsection{Frameworks for Understanding Computations}
The techniques discussed so far (probing, patching, ablation, SAEs, transcoders) provide tools to investigate specific components or representations. Frameworks for understanding computations aim to synthesize these findings into a more holistic view of how NNs perform tasks, often by identifying interconnected pathways or relating network operations to higher-level causal models.

\subsubsection{Circuit Analysis}
\textbf{Circuit Analysis} refers to the process of \textbf{understanding computational pathways involving multiple interconnected components} within a NN. The goal is often to identify a subgraph of the full network responsible for a specific capability or behavior. This typically involves \textbf{combining insights from multiple techniques}: observational methods like probing or SAEs might identify candidate components or features, while interventional techniques like activation patching, ablation, or causal tracing are used to confirm the causal roles of these components and map out their functional connections within the identified circuit. Circuit analysis moves beyond single-neuron or single-layer analysis to explain how information flows and is transformed through sequences or groups of network elements to achieve a particular outcome.

\subsubsection{Causal Abstraction}
\textbf{Causal Abstraction} provides a formal framework for relating the complex, low-level computations within a neural network to simpler, higher-level causal models. Its core idea is the \textbf{mapping of low-level neural network computations to higher-level causal graphs}, such as SCMs or DAGs often used in fields like bio-statistics (cf. Section~\ref{ssec:intro_scms_dags}). This framework aims to determine if the network's internal processing can be faithfully represented by a simpler causal model involving higher-level variables.

Let $f$ represent the neural network (the low-level system) operating on inputs $x$, producing internal states $h$ and outputs $y$. A causal abstraction proposes a high-level causal model $M_{HL}$ (e.g., an SCM) with variables $U, V, W, \dots$ and a mapping (abstraction function) $\alpha$ that connects the states of the low-level system to the states of the high-level variables (e.g., $\alpha(h)$ might determine the value of $V$). The key question is whether interventions performed on the low-level system $f$ produce effects consistent with the causal relationships defined in $M_{HL}$.

This framework directly \textbf{helps relate NN mechanisms to causal graphs used in bio-stats}. For instance, a DAG in bio-statistics might model the relationship between baseline covariates $W$, treatment $A$, and outcome $Y$. Causal abstraction attempts to find corresponding representations or computational pathways within the NN $f$ (trained, perhaps, as part of a TMLE estimator) that map to these variables $W, A, Y$ and asks if the network's internal computations respect the causal dependencies (e.g., $W \rightarrow A$, $W \rightarrow Y$, $A \rightarrow Y$) specified in the DAG.

\textbf{Interventions, particularly activation patching, are crucial within this framework for testing the faithfulness of the abstraction}. An intervention $do(V=v)$ in the high-level model $M_{HL}$ corresponds to interventions on the low-level network $f$. For example, using activation patching, we can force the network's internal state $h$ into a configuration $\tilde{h}$ such that $\alpha(\tilde{h})$ corresponds to the high-level state $V=v$. Let $f_{patched}$ denote the network under this intervention. The abstraction is considered faithful if the subsequent behavior of $f_{patched}$ aligns with the predictions of $M_{HL}$ under the intervention $do(V=v)$. For instance, if $M_{HL}$ posits that $V$ causes $Z$ but is independent of $X$ given its parents, then patching the network components corresponding to $V$ should affect the network outputs corresponding to $Z$, but ideally not those corresponding to $X$ (in a way not mediated by the parents). By systematically performing such interventions mirroring the causal structure of $M_{HL}$ and checking for consistency in the network's behavior, causal abstraction aims to validate whether the high-level causal model is a meaningful and accurate description of the network's underlying computational mechanisms.



\section{Synthetic Data Generation via Interpretable Manipulation of Predictive Model Internals}

\subsection{Motivation: Beyond Black-Box Generation for Causal Analysis}

The evaluation and refinement of causal inference methodologies, such as Targeted Maximum Likelihood Estimation (TMLE) within bio-statistics, necessitate access to data where the ground truth causal structures are known and controllable. Synthetic data generation serves this purpose, allowing researchers to rigorously test estimators under diverse scenarios, for instance, by systematically varying the strength of confounding between a treatment $A$ and an outcome $Y$ via covariates $W$, or by manipulating the degree of treatment effect heterogeneity across different patient subgroups defined by $W$.

Standard generative models, while powerful for capturing complex data distributions, often function as black-boxes themselves and present significant challenges for fine-grained, targeted control over specific causal parameters governing the data generating process. Modifying a specific aspect, like the influence of a single confounder $W_k$ on the treatment assignment mechanism $P(A|W)$, typically requires retraining the entire generative model, a computationally intensive and often impractical endeavor. There is a need for methods that permit more direct manipulation of the underlying causal relationships within the synthetic data generation process.

This work proposes leveraging predictive neural networks, potentially including those already trained as nuisance function estimators within a TMLE procedure (e.g., estimators for the conditional treatment assignment probability $g(A|W) = P(A|W)$ and the conditional outcome expectation $\bar{Q}(A,W) = E[Y|A,W]$), as the basis for synthetic data generation. These networks, through their training, implicitly learn representations of the conditional distributions governing the observed data. The core idea is to employ techniques from Mechanistic Interpretability (MI) not merely for understanding these networks, but to actively \textit{intervene} on their internal parameters (e.g., weights, attention scores) that represent specific causal pathways. By modifying these internal components, we aim to generate data from \textit{altered} conditional distributions, $P'(A|W)$ or $P'(Y|A,W)$, thereby achieving targeted control over the causal characteristics of the generated data without necessitating complete model retraining. This approach bridges the gap between the need for controlled synthetic benchmarks and the insights provided by MI into the functioning of predictive models.

\subsection{Approach: Conditional Data Generation Using Manipulated Internals}

The proposed approach circumvents the need to model and generate the full joint distribution $P(W, A, Y)$. Instead, it leverages the empirical distribution of baseline covariates $W$ from a real dataset and focuses on generating counterfactual treatments $A'$ and outcomes $Y'$ conditional on these observed covariates, using neural networks whose internal mechanisms have been purposefully manipulated.

\paragraph{Core Idea} We begin with a sample of baseline covariates $\{W_i\}_{i=1}^n$ drawn from their empirical distribution in a real dataset, $\hat{P}(W)$. We assume access to, or train, neural networks that model the key conditional distributions necessary for causal analysis: one network, $g_{net}$, estimating the treatment mechanism $P(A|W)$, and another network, $Q_{net}$, estimating relevant aspects of the conditional outcome distribution $P(Y|A,W)$, such as the conditional expectation $E[Y|A,W]$. These networks might be components previously trained for a Deep TMLE analysis or specifically trained for this generative task. Using MI techniques, we identify internal parameters within $g_{net}$ and $Q_{net}$ that correspond to specific causal influences (e.g., the effect of a confounder on treatment assignment, the main treatment effect on the outcome). We then create modified networks, $g'_{net}$ and $Q'_{net}$, by directly altering these identified parameters. Finally, we use these manipulated networks to sample new treatments $A'_i$ and outcomes $Y'_i$ conditional on the original $W_i$.

\paragraph{Process Outline} The procedure involves the following steps:

\subparagraph{Obtain Baseline Data} Utilize the observed baseline covariates $W$ from an existing real-world dataset. This anchors the synthetic data in realistic covariate structures and distributions, $\hat{P}(W)$.

\subparagraph{Train Predictive Components} Train or obtain pre-trained neural networks $g_{net}(\cdot | W)$ approximating $P(A|W)$ and $Q_{net}(\cdot | A, W)$ approximating $E[Y|A,W]$ (or potentially $P(Y|A,W)$ if generating the full conditional distribution is feasible). These networks implicitly encode the conditional relationships learned from the real data.

\subparagraph{MI-Guided Identification} Apply core MI techniques (detailed in Section 4.2) to $g_{net}$ and $Q_{net}$. The objective is to pinpoint specific internal components—such as individual weights, groups of weights corresponding to specific connections, neuron activation patterns, or attention scores in Transformer-based models—that are causally responsible for encoding the particular causal relationship targeted for modification. For example, identify the parameters in $g_{net}$ mediating the influence of a specific confounder $W_k$ on the prediction of $A$, or the parameters in $Q_{net}$ primarily responsible for representing the main effect of $A$ on the prediction of $Y$.

\subparagraph{Targeted Weight Manipulation} Create modified network instances $g'_{net}$ and $Q'_{net}$ by directly intervening on the parameters identified in the previous step. This manipulation is the core interpretability-driven intervention. Examples include: scaling specific weights or weight matrices to increase or decrease the strength of a particular influence (e.g., amplify confounding), setting specific weights to zero to remove an influence (e.g., eliminate a direct effect pathway), or modifying attention patterns to change how information from different inputs is integrated.

\subparagraph{Conditional Sampling} For each baseline covariate vector $W_i$ from the real dataset:
\begin{enumerate}
    \item Sample a counterfactual treatment $A'_i \sim P'(A|W_i)$ using the manipulated treatment mechanism network $g'_{net}(A|W_i)$. The output of $g'_{net}$ (e.g., a probability for binary $A$) defines the sampling distribution.
    \item Sample a counterfactual outcome $Y'_i \sim P'(Y|A'_i, W_i)$ using the manipulated outcome network $Q'_{net}(Y|A'_i, W_i)$. This step requires careful consideration of $Q_{net}$'s output. If $Q'_{net}$ outputs the conditional expectation $E'[Y|A'_i, W_i]$, we must make an assumption about the conditional distribution to enable sampling. For instance, for a binary outcome $Y$, we can sample $Y'_i \sim \text{Bernoulli}(p=E'[Y|A'_i, W_i])$. For a continuous outcome, we might sample $Y'_i \sim \mathcal{N}(\mu=E'[Y|A'_i, W_i], \sigma^2=\hat{\sigma}^2)$, where $\hat{\sigma}^2$ is a fixed estimate of the residual variance, possibly obtained from the original $Q_{net}$ fit or the data.
\end{enumerate}

\subparagraph{Construct Synthetic Dataset} Combine the original baseline covariates $W_i$ with the newly generated counterfactual treatments $A'_i$ and outcomes $Y'_i$ to form the final synthetic dataset $\mathcal{D}' = \{(W_i, A'_i, Y'_i)\}_{i=1}^n$. This dataset reflects the original covariate structure but incorporates the specific causal modifications introduced via the MI-guided manipulation of the network internals.


\subsection{Techniques for Identifying and Modifying Causal Pathways}

The effectiveness of the proposed conditional data generation approach hinges on the ability of Mechanistic Interpretability (MI) techniques to accurately identify the specific internal components of the networks $g_{net}$ and $Q_{net}$ responsible for encoding the targeted causal relationships, and subsequently enabling precise modifications to these components.

\paragraph{Finding Causal Pathways} Several MI techniques can be employed to trace and quantify the influence of specific inputs or intermediate representations on the network's output, thereby identifying the pathways encoding causal effects:

\subparagraph{Activation Patching / Interchange Interventions} This technique (cf. Section 4.2.2) is particularly well-suited for pinpointing causal links within the network. To identify the pathway mediating the effect of a confounder $W_k$ on treatment assignment $A$ within $g_{net}$, one could run the network on two sets of inputs: one where $W_k$ has a 'high' value and another where it has a 'low' value (while keeping other covariates similar). By systematically swapping activation vectors at different layers or components between these runs and observing the change in the predicted $P(A|W)$, we can locate the specific components (e.g., attention heads, MLP layers) through which $W_k$'s influence flows. Similarly, in $Q_{net}$, patching activations related to the treatment input $A$ between runs corresponding to hypothetical treated ($A=1$) and control ($A=0$) scenarios can reveal the components mediating the main treatment effect on the outcome prediction $E[Y|A,W]$.

\subparagraph{Gradient-based Attribution} Methods like Integrated Gradients or simple saliency maps can provide an initial assessment of which input features (e.g., specific confounders $W_k$) or internal neurons have the most significant influence on the final output prediction (e.g., $P(A|W)$ for $g_{net}$ or $E[Y|A,W]$ for $Q_{net}$). While primarily correlational, high gradient attribution can suggest components worth investigating further with interventional techniques like patching.

\subparagraph{Circuit Analysis} For more complex relationships, particularly in deeper networks or Transformers, understanding the computational pathway might involve combining multiple techniques (cf. Section 4.2.5). This could involve tracing the flow of information related to a specific confounder $W_k$ through attention layers (identified via patching head activations) and subsequent MLP layers (identified via patching MLP activations or using weight analysis) within $g_{net}$ or $Q_{net}$.

\paragraph{Interpreting Learned Features (e.g., via SAEs)} If techniques like Sparse Autoencoders (SAEs) (cf. Section 4.2.4) are used to decompose the internal activations of $g_{net}$ or $Q_{net}$ into potentially monosemantic features, MI can shift towards identifying specific learned features that correspond to relevant concepts. For instance, one might find an SAE feature in $g_{net}$'s activations that strongly correlates with a particular confounder $W_k$. Interventions can then target the network's interaction with this interpretable feature, such as modifying the weights that read from this feature dimension into later layers, providing a more conceptually grounded way to manipulate the encoded information.

\paragraph{Implementing Modifications} Once MI techniques have identified the relevant network components (weights, neurons, attention heads, SAE features) constituting a causal pathway, the modification step translates the desired causal change into a concrete intervention on these components to create $g'_{net}$ and $Q'_{net}$:

\subparagraph{Parameter Scaling} This is often the most direct approach. If a specific weight matrix entry, a neuron's output weight, or an attention score is identified by MI as mediating the strength of influence (e.g., the weight connecting the representation of $W_k$ to the logit predicting $A$ in $g_{net}$), this parameter can be directly multiplied by a scalar factor. Scaling it above 1 increases the influence (e.g., strengthens confounding or treatment effect), while scaling it towards 0 decreases the influence.

\subparagraph{Ablation} To completely remove a specific causal influence represented by an identified component or pathway, ablation can be used (cf. Section 4.2.2). This involves setting the identified weights or activations to zero (or a neutral baseline value). For example, ablating the attention head primarily responsible for attending from the treatment token $A$ to the output prediction in $Q_{net}$ could simulate removing the direct treatment effect.

\subparagraph{Targeted Edits} For features identified via methods like SAEs, modifications might involve altering the weights that write information into that feature dimension or the weights that read information out from it, thereby controlling how the network utilizes that specific concept (e.g., the identified confounder feature).

The choice of modification technique depends on the desired outcome (e.g., amplification, reduction, removal of an effect) and the nature of the components identified by the MI analysis. The goal is always to perform a targeted, interpretable change to the network's parameters that directly corresponds to the intended modification of the underlying causal structure.

\subsection{Proof-of-Concept: Modifying Confounding and Treatment Effect in a Static Setting}

To demonstrate the feasibility and effectiveness of generating synthetic data with controlled causal characteristics using MI-guided interventions, we outline a proof-of-concept experiment in a simple, static (single time point) setting. The goal is to independently modify the strength of confounding and the magnitude of the average treatment effect (ATE) in a generated dataset.

\paragraph{Experimental Setup} We assume a standard observational data structure $(W, A, Y)$, where $W = (W_1, \dots, W_p)$ are baseline covariates, $A$ is a binary treatment, and $Y$ is an outcome (e.g., continuous or binary). We will first simulate or use a real dataset to train initial predictive networks. For simplicity, we utilize Multi-Layer Perceptrons (MLPs) for both the treatment mechanism and outcome expectation networks.

\subparagraph{Train Base Networks}
First, train two simple MLP networks on an initial dataset (either simulated with known properties or a real dataset):
\begin{itemize}
    \item $g_{net}$: An MLP trained to predict the probability of treatment given covariates, $P(A=1|W)$. The output layer uses a sigmoid activation.
    \item $Q_{net}$: An MLP trained to predict the conditional expectation of the outcome given treatment and covariates, $E[Y|A,W]$. The output activation depends on the nature of $Y$ (e.g., linear for continuous $Y$, sigmoid for binary $Y$ interpreted as $P(Y=1|A,W)$).
\end{itemize}
We denote the parameters (weights and biases) of these trained networks as $\theta_g$ and $\theta_Q$.

\paragraph{Scenario 1: Modify Confounding Strength}
The objective is to generate datasets where the association between a specific strong confounder, say $W_1$, and the treatment assignment $A$ is artificially increased or decreased, while the true underlying treatment effect on the outcome remains unchanged.

\subparagraph{MI Identification (Confounding Pathway)} Apply MI techniques to the trained $g_{net}$ to identify the parameters primarily responsible for mediating the influence of input $W_1$ on the output $P(A=1|W)$. In a simple MLP, this might involve examining the weights in the first hidden layer connected to the input neuron for $W_1$, or using gradient attribution to confirm $W_1$'s influence and trace it through the network. Let the identified set of parameters be $\theta_{g, W_1 \to A} \subset \theta_g$.

\subparagraph{Manipulation (Create $g'_{net}$)} Create modified parameter sets $\theta'_{g, \alpha}$ by scaling the identified confounding parameters $\theta_{g, W_1 \to A}$ by a factor $\alpha$. For instance, multiply the relevant weights by $\alpha$. Setting $\alpha > 1$ aims to increase confounding, $0 \le \alpha < 1$ aims to decrease it, and $\alpha = 0$ aims to remove $W_1$'s direct influence on $A$ through this pathway. Let $g'_{net, \alpha}$ denote the network with parameters $\theta'_{g, \alpha}$.

\subparagraph{Data Generation (Modified Confounding)} Using a set of baseline covariates $\{W_i\}_{i=1}^n$ from the original data:
\begin{enumerate}
    \item For each $W_i$, sample $A'_i \sim \text{Bernoulli}(p = g'_{net, \alpha}(A=1|W_i))$.
    \item For each $(W_i, A'_i)$, predict $E[Y|A'_i, W_i]$ using the \textit{original} outcome network $Q_{net}$. Sample $Y'_i$ based on this expectation (e.g., $Y'_i \sim \mathcal{N}(Q_{net}(A'_i, W_i), \hat{\sigma}^2)$ for continuous $Y$).
\end{enumerate}
This yields a dataset $\mathcal{D}'_{\text{confound}, \alpha} = \{(W_i, A'_i, Y'_i)\}$.

\subparagraph{Verification} Estimate the ATE on $\mathcal{D}'_{confound, \alpha}$. Since $Q_{net}$ was unchanged, the true ATE in the generated data should be constant regardless of $\alpha$. However, calculate the naive association measure $\Delta_{naive} = E[Y'|A'=1] - E[Y'|A'=0]$ (simple difference in means between treated and untreated groups in $\mathcal{D}'_{confound, \alpha}$). We expect the bias, $|\Delta_{naive} - \text{ATE}|$, to vary systematically with $\alpha$, increasing for $\alpha > 1$ and decreasing for $\alpha < 1$, demonstrating successful manipulation of the confounding strength.

\paragraph{Scenario 2: Modify Treatment Effect Magnitude}
The objective is to generate datasets where the true ATE is artificially scaled, while the confounding structure remains as in the original data.

\subparagraph{MI Identification (Treatment Effect Pathway)} Apply MI techniques to the trained $Q_{net}$ to identify the parameters primarily responsible for mediating the influence of the treatment input $A$ on the output $E[Y|A,W]$. In an MLP, this could involve weights connected to the input neuron for $A$, or analysis of how representations differ between $A=1$ and $A=0$ inputs using techniques like activation patching. Let the identified set of parameters be $\theta_{Q, A \to Y} \subset \theta_Q$.

\subparagraph{Manipulation (Create $Q'_{net}$)} Create modified parameter sets $\theta'_{Q, \beta}$ by applying a scaling factor $\beta$ to the identified treatment effect parameters $\theta_{Q, A \to Y}$. For example, scale the weights representing the main effect of $A$. Let $Q'_{net, \beta}$ denote the network with parameters $\theta'_{Q, \beta}$.

\subparagraph{Data Generation (Modified Effect)} Using the baseline covariates $\{W_i\}_{i=1}^n$:
\begin{enumerate}
    \item For each $W_i$, sample $A'_i \sim \text{Bernoulli}(p = g_{net}(A=1|W_i))$ using the \textit{original} treatment network $g_{net}$.
    \item For each $(W_i, A'_i)$, predict $E'[Y|A'_i, W_i]$ using the \textit{manipulated} outcome network $Q'_{net, \beta}$. Sample $Y'_i$ based on this modified expectation.
\end{enumerate}
This yields a dataset $\mathcal{D}'_{\textit{effect}, \beta} = \{(W_i, A'_i, Y'_i)\}$.

\subparagraph{Verification} Estimate the ATE' on the generated dataset $\mathcal{D}'_{effect, \beta}$. Since the ground truth (manipulated) nuisance functions $g_{net}$ and $Q'_{net, \beta}$ are effectively known for the generated data, a reliable estimate of ATE' can be obtained (e.g., using TMLE with these networks, or direct standardization/G-computation). Verify that the estimated ATE' changes approximately proportionally to the scaling factor $\beta$. For instance, if the original ATE was $\psi_0$, the ATE' in the data generated with scaling factor $\beta$ should be close to $\psi_0 \times \beta$ (or a similar predictable relationship depending on how the scaling was implemented).

This proof-of-concept experiment, using simple models and targeted manipulations identified via MI, serves to validate the core principle: that interventions on the internal parameters of predictive networks allow for the generation of synthetic data with specific, controllably modified causal characteristics.


\paragraph{Scenario 3: Parametric Mimicry of Weighting via Cross-Network Intervention}

This scenario explores a more speculative use of MI, attempting to directly modify the parameters of the outcome network ($Q_{net}$) to parametrically mimic an effect similar to weighting or adjustment, guided by the structure learned by the treatment network ($g_{net}$). This differs fundamentally from standard IPW (which weights samples) and TMLE (which adjusts predictions based on propensity scores).

\subparagraph{Objective} To investigate if identifying parameters in $g_{net}$ associated with confounding and intervening on *structurally corresponding* parameters in $Q_{net}$ can lead to a modified outcome prediction function that implicitly corrects for some of the confounding bias, when estimating the ATE via direct standardization using the manipulated $Q'_{net}$.

\subparagraph{Crucial Assumption} This scenario critically assumes that $g_{net}$ and $Q_{net}$ possess \textbf{identical network architectures} (same layers, dimensions, activation functions, etc.). This allows for a direct positional mapping of parameters between the two networks, even if they were trained separately and learned different functions.

\subparagraph{MI Identification (Confounding Pathway in $g_{net}$)} As in Scenario 1, apply MI techniques to the trained $g_{net}$ to identify the set of parameters $\theta_{g, W_1 \to A} \subset \theta_g$ primarily responsible for mediating the influence of a strong confounder $W_1$ on the treatment prediction $P(A=1|W)$.

\subparagraph{Parameter Mapping (Heuristic)} Based on the identical architecture assumption, identify the set of parameters $\theta_{Q, corresp}$ within $Q_{net}$ that are located at the \textit{exact same positions} (e.g., same layer index, same weight indices within that layer's matrix/vector) as the parameters $\theta_{g, W_1 \to A}$ identified in $g_{net}$. This is a strong heuristic, assuming that parameters in similar structural locations might play analogous (though functionally different) roles related to $W_1$ in their respective networks.

\subparagraph{Manipulation (Create $Q'_{net}$)} Create a modified outcome network $Q'_{net, \gamma}$ by intervening on the corresponding parameters $\theta_{Q, corresp}$. The nature of the intervention here is exploratory. For instance, one might scale these parameters by a factor $\gamma$, potentially aiming to dampen ($\gamma < 1$) or amplify ($\gamma > 1$) the way $Q_{net}$ utilizes information related to $W_1$ through these specific pathways. The choice of $\gamma$ might even be informed by the magnitude of the effect observed in $g_{net}$, although the functional relationship is unclear. Let the modified parameters be $\theta'_{Q, \gamma}$.

\subparagraph{Data Generation (Parametric Adjustment Simulation)} Using the baseline covariates $\{W_i\}_{i=1}^n$:
\begin{enumerate}
    \item For each $W_i$, sample $A'_i \sim \text{Bernoulli}(p = g_{net}(A=1|W_i))$ using the \textit{original} treatment network $g_{net}$. The confounding structure in the treatment assignment remains unchanged.
    \item For each $(W_i, A'_i)$, predict the outcome expectation $E'[Y|A'_i, W_i]$ using the \textit{manipulated} outcome network $Q'_{net, \gamma}$. Sample $Y'_i$ based on this modified expectation (e.g., $Y'_i \sim \mathcal{N}(Q'_{net, \gamma}(A'_i, W_i), \hat{\sigma}^2)$).
\end{enumerate}
This yields a dataset $\mathcal{D}'_{param\_ipw, \gamma} = \{(W_i, A'_i, Y'_i)\}$.

\subparagraph{Verification} The key verification is whether this parametric intervention reduces bias compared to using the original $Q_{net}$.
\begin{enumerate}
    \item Estimate an ATE proxy using direct standardization (G-computation) based on the manipulated network: $\hat{\psi}_{param, \gamma} = \frac{1}{n} \sum_{i=1}^n [Q'_{net, \gamma}(A=1, W_i) - Q'_{net, \gamma}(A=0, W_i)]$.
    \item Compare this $\hat{\psi}_{param, \gamma}$ to the ATE proxy obtained using the original outcome network: $\hat{\psi}_{orig} = \frac{1}{n} \sum_{i=1}^n [Q_{net}(A=1, W_i) - Q_{net}(A=0, W_i)]$.
    \item Compare both estimates to the true ATE ($\psi_0$), if known (e.g., if the initial data was simulated).
    \item The hypothesis is whether there exists a manipulation factor $\gamma$ such that the bias $|\hat{\psi}_{param, \gamma} - \psi_0|$ is smaller than the bias $|\hat{\psi}_{orig} - \psi_0|$. Can we systematically reduce the bias inherent in the original $Q_{net}$'s predictions by modifying parameters identified via $g_{net}$?
\end{enumerate}
This scenario tests the potential for transferring structural information identified via MI across networks with identical architectures to perform a novel, albeit heuristic, form of bias adjustment directly within the network parameters. Its success would depend strongly on the extent to which the heuristic mapping assumption holds and whether the chosen intervention on $\theta_{Q, corresp}$ appropriately counteracts the confounding effects implicitly learned by $Q_{net}$. It is important to note that this approach lacks the theoretical guarantees of established methods like IPW or TMLE.

\paragraph{Scenario 3: Heuristic Parametric "Correction" via Shared Weights (MTL)}
This scenario explores the speculative idea of using MI across components of a Multi-Task Learning (MTL) network to perform a parameter-level intervention intended to mimic bias adjustment.

\subparagraph{MTL Setup} Train a network with shared parameters $\theta_{shared}$ for the initial layers processing $W$, and separate heads for treatment prediction ($\theta_{g\_head}$) and outcome prediction ($\theta_{Q\_head}$). This yields initial estimators $\hat{g}(W; \hat{\theta}_{shared}, \hat{\theta}_{g\_head})$ and $\hat{\bar{Q}}(A, W; \hat{\theta}_{shared}, \hat{\theta}_{Q\_head})$.

\subparagraph{MI Identification \& Heuristic Intervention} Use MI techniques on the components defining $\hat{g}$ (i.e., $\hat{\theta}_{shared}$ and $\hat{\theta}_{g\_head}$) to identify pathways/parameters within $\hat{\theta}_{shared}$ strongly associated with the influence of a confounder $W_1$ on the prediction $\hat{g}$. Let this subset be $\theta_{shared, W_1 \to A}$. Then, perform a heuristic intervention directly on these shared parameters, creating $\theta'_{shared, \gamma} = \hat{\theta}_{shared} + \Delta\theta_{shared, \gamma}$, where the modification $\Delta\theta_{shared, \gamma}$ (e.g., scaling the identified parameters by $\gamma$) is based solely on the analysis of the $g$-pathway. The intuition (though flawed) is to adjust the shared representation itself to somehow account for the confounding identified via $g_{net}$.

\subparagraph{Data Generation \& Estimation} Generate a dataset $\mathcal{D}'_{heuristic, \gamma} = \{(W_i, A'_i, Y'_i)\}$ where $A'_i$ is sampled using the original $\hat{g}$ (or potentially the modified $g'$) and $Y'_i$ is sampled based on predictions from the modified outcome network $Q'_{net, \gamma}(A, W) = Q_{net}(A, W; \theta'_{shared, \gamma}, \hat{\theta}_{Q\_head})$. Estimate the ATE using G-computation on the modified outcome network: $\hat{\psi}_{heuristic, \gamma} = P_n [Q'_{net, \gamma}(1,W) - Q'_{net, \gamma}(0,W)]$.

\subparagraph{Discussion} This scenario attempts a novel form of cross-network parameter influence. However, it is **highly heuristic and lacks theoretical guarantees** for consistency or double robustness regarding the ATE estimate $\hat{\psi}_{heuristic, \gamma}$. Key issues include:
    \begin{itemize}
        \item The mapping of parameter function between the $g$-pathway and the $Q$-pathway within $\theta_{shared}$ is not formally established.
        \item The intervention $\Delta\theta_{shared, \gamma}$ is not derived from principles known to satisfy the EIC equation or target ATE bias reduction (like the TMLE fluctuation step).
        \item Choosing an optimal $\gamma$ is problematic without ground truth or a theoretical objective.
        \item It bypasses the explicit use of the estimated propensity score function $\hat{g}(W)$ required by established robust methods.
    \end{itemize}
While potentially interesting for exploring internal network dynamics, this approach does not currently provide a sound basis for causal effect estimation.

\paragraph{Scenario 4: Robust Estimation using MTL Outputs within Standard Frameworks}
This scenario represents the theoretically grounded way to leverage the MTL architecture from Scenario 3 for robust causal inference.

\subparagraph{MTL Setup} Train the same MTL network as in Scenario 3, obtaining initial nuisance function estimates $\hat{g}(W)$ and $\hat{\bar{Q}}(A, W)$ from the respective heads.

\subparagraph{No Parameter Intervention} Do not perform any MI-guided intervention on the network parameters $\hat{\theta}_{shared}, \hat{\theta}_{g\_head}, \hat{\theta}_{Q\_head}$ after initial training.

\subparagraph{Estimation via Established Methods} Use the network *outputs* $\hat{g}$ and $\hat{\bar{Q}}$ as the initial nuisance function estimates within a standard, theoretically validated causal inference framework:
    \begin{itemize}
        \item **TMLE:** Apply the standard TMLE algorithm (fluctuation step using clever covariate based on $\hat{g}$, update $\hat{\bar{Q}}$ to $\hat{\bar{Q}}^*$, average predictions).
        \item **AIPW:** Compute the Augmented Inverse Probability Weighted estimator using $\hat{g}$ and $\hat{\bar{Q}}$.
    \end{itemize}
Let the resulting estimator be $\hat{\psi}_{MTL-TMLE}$ or $\hat{\psi}_{MTL-AIPW}$.

\subparagraph{Discussion} This approach **inherits the standard theoretical guarantees** (consistency, double robustness, asymptotic normality under standard regularity conditions) of TMLE or AIPW. The potential advantage of the MTL architecture here is practical, not theoretical in terms of guarantees: the shared training *might* produce initial estimates $\hat{g}$ and $\hat{\bar{Q}}$ that are more accurate or efficient (especially in finite samples) than estimates obtained from separately trained networks. Better initial estimates can lead to more stable and efficient final TMLE/AIPW estimates, even though the asymptotic guarantees rely only on consistency conditions. This scenario represents the current best practice for leveraging advanced NN architectures like MTL for robust causal effect estimation. It uses NNs for flexible nuisance function estimation within a framework that provides formal guarantees.

\subsection{Extension to Longitudinal Data}

% Extending the MI-driven synthetic data generation approach to longitudinal settings, where data arrives as sequences $(W_{i,t}, A_{i,t}, Y_{i,t})$ over time $t=0, \dots, T$, introduces complexities related to temporal dependencies and time-varying confounding. Here, covariates $W_t$ can be influenced by past treatments $A_{<t}$ and also confound the effect of future treatments $A_{\ge t}$ on outcomes $Y_{\ge t}$. Estimating causal effects in such settings often requires sophisticated methods like Longitudinal TMLE (LTMLE), and correspondingly, evaluating these methods demands synthetic data capturing these dynamic relationships.

% The nuisance functions in longitudinal settings are inherently sequential. For instance, the treatment mechanism at time $t$ depends on the history of past treatments and covariates, $P(A_t | \bar{A}_{t-1}, \bar{W}_t)$, and the outcome expectation depends on the history up to time $t$, $E[Y_t | \bar{A}_t, \bar{W}_t]$, where $\bar{X}_t = (X_0, \dots, X_t)$. Consequently, the networks $g_{net,t}$ and $Q_{net,t}$ used for initial estimation (and potentially for generation) must be sequence models capable of handling such historical dependencies. As exemplified by recent work like [Shirakawa et al., 2024], Transformer architectures are increasingly employed for this purpose within the LTMLE framework due to their ability to capture long-range dependencies via attention mechanisms.

% Applying the MI-driven generation approach in this context involves adapting the identification and manipulation steps to these sequence models:

% \paragraph{MI Target Identification in Sequence Models (Transformers)}
% When using Transformer-based models for $g_{net,t}$ and $Q_{net,t}$, MI techniques focus on dissecting the components responsible for processing temporal information:
% \subparagraph{Attention Mechanisms} Activation patching or gradient analysis can be applied to attention heads. Key targets include:
% \begin{itemize}
%     \item In $g_{net,t}$: Identifying attention scores between the input representing the current prediction time $t$ and inputs representing past covariates $W_{t-k}$ versus past treatments $A_{t-k}$. This helps understand how strongly the model relies on specific historical factors, particularly confounders affected by past treatments, when predicting $A_t$.
%     \item In $Q_{net,t}$: Identifying attention scores between the input representation for the current outcome prediction $Y_t$ and the input for the current treatment $A_t$ versus inputs representing past history $(\bar{A}_{t-1}, \bar{W}_t)$. This reveals how the model weighs contemporaneous treatment information against historical context.
% \end{itemize}
% \subparagraph{Feed-Forward Network (FFN) Layers} Within each Transformer block, FFN layers process the information aggregated by the attention mechanism. MI techniques (patching, weight analysis) can identify FFN components specialized in processing specific information streams, such as those primarily handling treatment-related inputs or specific time-varying covariate information.

% \paragraph{Manipulation Examples in Longitudinal Settings}
% Based on the identified components, targeted manipulations can be designed to alter specific longitudinal causal dynamics:
% \subparagraph{Modifying Time-Varying Confounding Strength} If MI identifies attention patterns or FFN weights in $g_{net,t}$ that strongly link past treatments $A_{<t}$ to the representation of a current time-varying confounder $W_{k,t}$ (which in turn influences $A_t$), these pathways can be scaled. Increasing their strength would amplify the time-varying confounding induced by that pathway in the generated $A'_t$ sequence.
% \subparagraph{Altering Time-Varying Treatment Effect} In $Q_{net,t}$, if MI pinpoints attention heads or FFN components responsible for processing the current treatment $A_t$'s influence on $Y_t$, the corresponding weights can be scaled differently at different time steps $t$. This allows generating $Y'_t$ sequences where the treatment effect magnitude changes over time according to a specified pattern (e.g., diminishing effect, increasing effect).

% \paragraph{Goal: Controlled Longitudinal Dynamics}
% The objective is to generate sequences $(W_{i,t}, A'_{i,t}, Y'_{i,t})$, starting from real baseline data $W_{i,0}$ and potentially using observed intermediate covariates $W_{i,t}$ (if not modeling their generation explicitly), where the generated $A'_{i,t}$ and $Y'_{i,t}$ reflect specific, controlled modifications to the underlying causal structure. This could involve generating data with precisely amplified or reduced time-varying confounding, or with a known functional form for the evolution of the treatment effect over time. Such datasets are invaluable for systematically evaluating the performance and robustness of longitudinal causal inference methods like LTMLE under challenging, yet controlled, dynamic scenarios derived from real-world data complexities.

The principles of MI-guided synthetic data generation can be extended to the more complex longitudinal setting, where data consists of sequences of covariates, treatments, and outcomes over time, denoted as $(\bar{W}_T, \bar{A}_T, \bar{Y}_T)$, where $\bar{X}_t = (X_0, \dots, X_t)$. Longitudinal data introduces challenges such as time-varying confounding, where a variable $W_t$ can be both a confounder for the effect of $A_t$ on $Y_t$ and also affected by past treatments $A_{t-k}$. Methods like Longitudinal TMLE (LTMLE) are designed to handle these complexities, relying on estimates of time-varying nuisance functions, typically the conditional probability of treatment $g_t(A_t | \bar{A}_{t-1}, \bar{W}_t) = P(A_t | \bar{A}_{t-1}, \bar{W}_t)$ and the conditional expectation of the outcome $\bar{Q}_t( \bar{A}_t, \bar{W}_t) = E[Y_t | \bar{A}_t, \bar{W}_t]$ (or related quantities).

\paragraph{Modeling Longitudinal Dependencies} Neural network architectures adept at sequence modeling are required to capture the temporal dependencies inherent in $g_t$ and $\bar{Q}_t$. Recurrent Neural Networks (RNNs) like LSTMs (cf. Section 2.4.2) were traditional choices, but Transformer architectures (cf. Section 2.3.3) have shown significant promise due to their attention mechanism's ability to capture long-range dependencies effectively, as explored in contexts like LTMLE by [Shirakawa et al., 2024]. We can consider Transformer-based models, denoted $g_{net, T}$ and $Q_{net, T}$, trained to estimate the sequences of treatment probabilities and outcome expectations, respectively, possibly using shared components to represent the history $(\bar{A}_{t-1}, \bar{W}_t)$.

\paragraph{MI Target Identification in Sequential Models} Identifying causal pathways within these sequential models requires adapting MI techniques:
\subparagraph{Attention Mechanism Analysis} The attention scores within Transformers are prime targets for MI. We can investigate:
\begin{itemize}
    \item How strongly specific past treatments $A_{t-k}$ or covariates $W_{t-j}$ attend to the representation used to predict the current treatment $A_t$ in $g_{net, T}$. This reveals how the network models the influence of history on current treatment decisions, including time-varying confounding pathways.
    \item How strongly the current treatment representation $A_t$ attends to the representation used for predicting the current outcome $Y_t$ (or future outcomes) in $Q_{net, T}$. This helps isolate the component representing the instantaneous or lagged treatment effect.
    \item Attention patterns related to specific covariates $W_t$ influencing $A_t$ or $Y_t$.
\end{itemize}
Activation patching can be applied to attention outputs or specific head outputs to quantify the causal effect of attending to specific past elements.

\subparagraph{FFN Layer Analysis} The feed-forward network (FFN) blocks within Transformer layers process information aggregated by the attention mechanism. MI techniques like weight analysis or patching activations within these FFN layers can identify how information about specific variables (e.g., the current treatment $A_t$) is transformed and utilized for prediction.

\paragraph{Manipulation Examples in Longitudinal Setting} Targeted manipulations can now address dynamic aspects:
\begin{itemize}
    \item \textbf{Modifying Feedback:} Alter attention scores or weights in $g_{net, T}$ connecting past treatments $A_{t-k}$ to the prediction of $A_t$ (potentially via intermediate $W_t$ representations if explicitly modeled) to strengthen or weaken the feedback loops characteristic of time-varying confounding affected by past treatment.
    \item \textbf{Altering Time-Varying Treatment Effect:} Scale weights within the FFN layers of $Q_{net, T}$ that process the representation of the current treatment $A_t$, identified via MI as mediating its effect on $Y_t$. This allows scaling the magnitude of the treatment effect specifically at time $t$, potentially even making the scaling factor itself time-dependent.
    \item \textbf{Changing Confounding Dynamics:} Modify attention patterns or weights related to how a specific time-varying confounder $W_t$ influences the prediction of $A_t$ at each step $t$, altering the instantaneous confounding relationship over time.
\end{itemize}

\paragraph{Sequential Data Generation} Generating longitudinal data involves iterating through time steps. Starting with baseline covariates $W_0$ (and potentially $Y_0$ if relevant) from real data:
\begin{enumerate}
    \item For $t = 0, \dots, T-1$:
        \item Given the generated history $(\bar{A}'_{t-1}, \bar{W}'_t)$, sample the next treatment $A'_t \sim P'(A_t | \bar{A}'_{t-1}, \bar{W}'_t)$ using the manipulated treatment mechanism network $g'_{net, T}$.
        \item Given the history including the new treatment $(\bar{A}'_t, \bar{W}'_t)$, predict the outcome expectation $E'[Y_t | \bar{A}'_t, \bar{W}'_t]$ using the manipulated outcome network $Q'_{net, T}$.
        \item Sample the outcome $Y'_t$ based on the prediction (e.g., $Y'_t \sim \text{Bernoulli}(E'[Y_t | \dots])$).
        \item (Optional) If time-varying covariates $W_{t+1}$ are also being generated based on history, sample $W'_{t+1}$ using a separate manipulated network. Otherwise, use the observed $W_{t+1}$ from the real data if appropriate for the target parameter.
\end{enumerate}
This produces a synthetic longitudinal dataset $\mathcal{D}'_{long} = \{( \bar{W}'_{i,T}, \bar{A}'_{i,T}, \bar{Y}'_{i,T} )\}_{i=1}^n$.

\paragraph{Goal} The aim of this extension is to generate realistic longitudinal datasets where complex dynamic causal features, such as the strength of feedback loops or the evolution of treatment effects over time, are precisely controlled. Such datasets are invaluable for rigorously evaluating the performance of sophisticated causal inference methods like LTMLE under challenging, yet well-understood, conditions derived from modifications to networks trained on real-world temporal dynamics.

\subsection{Value Proposition: Controlled, Realistic Data for ATE Estimation}


The proposed methodology, leveraging Mechanistic Interpretability (MI) to manipulate predictive neural networks for conditional data generation, offers significant advantages for the development, testing, and validation of causal inference techniques, particularly in bio-statistical settings.

\paragraph{Targeted Control over Causal Mechanisms} Unlike standard generative models where modifying specific underlying causal parameters (like the exact strength of confounding by a variable $W_k$, or the magnitude of an interaction effect between $A$ and $W_j$) is often intractable without retraining, this approach enables precise, targeted interventions. By identifying and altering the specific internal components of pre-trained networks ($g_{net}, Q_{net}$) that encode these relationships, researchers gain fine-grained control over the causal structure of the generated data ($A', Y'$). This allows for the creation of datasets tailored to test specific hypotheses about estimator performance under known conditions.

\paragraph{Realistic Data Complexity} The generation process is anchored in real-world data. It utilizes the empirical distribution of baseline covariates $\hat{P}(W)$ and relies on predictive models ($g_{net}, Q_{net}$) trained on actual observational data. These networks implicitly capture the complex, potentially non-linear relationships and high-dimensional interactions present in the source data. Consequently, the generated conditional distributions $P'(A|W)$ and $P'(Y|A,W)$, while modified in targeted ways, retain a level of realism often absent in purely simulation-based studies that rely on simplified parametric assumptions for the data generating process. The generated data thus presents a more challenging and representative testbed for causal methods.

\paragraph{Systematic Evaluation of Causal Estimators} This framework provides an invaluable tool for the rigorous evaluation of causal inference estimators like TMLE, LTMLE, IPW, G-computation, and others. Researchers can generate multiple datasets where, for example, the degree of confounding is incrementally increased, the treatment effect heterogeneity follows a known pattern, or specific causal assumptions (like positivity violations introduced via manipulation of $g_{net}$) are violated in controlled ways. Assessing estimator performance (bias, variance, confidence interval coverage) across these systematically varied, realistic datasets allows for a deeper understanding of their strengths, weaknesses, and robustness under conditions derived from real data complexity but with known ground-truth modifications.

\paragraph{Powerful Validation Loop for Mechanistic Interpretability} The process serves as a crucial validation mechanism for the MI techniques themselves. The core premise is that if MI correctly identifies the network components responsible for a specific causal influence, then manipulating those components should lead to predictable changes in the causal structure of the generated data. For instance, if MI suggests certain weights in $Q_{net}$ encode the main treatment effect, scaling those weights by a factor of $\alpha$ should result in a generated dataset where the estimated ATE (using a reliable method like TMLE on the synthetic data $\mathcal{D}'$) is approximately $\alpha$ times the original ATE. Successfully demonstrating such expected changes provides strong evidence supporting the validity of the MI interpretation. Conversely, if the manipulation does not yield the anticipated causal shift in the generated data, it indicates limitations in the MI analysis, prompting refinement of the interpretability techniques. This creates a powerful feedback loop between understanding network mechanisms and verifying that understanding through controlled generation experiments.


\section{Mechanistic Interpretability as a Proxy Learning Toolkit}\label{sec:mi_proxy_learning_tk}

* Defining "Proxy Learning" in this Context: Explicitly state that given the complexity, full mechanistic understanding is often infeasible. MI techniques act as proxies – tools that allow us to assess specific aspects of the model's internal reasoning (feature encoding, causal reliance, alignment with known factors) without needing a complete computational graph understanding. These proxy insights help achieve the goals outlined in 4.1.
* The Toolkit Approach: Frame the techniques from 4.2 as a synergistic toolkit. No single technique gives the full picture.
* Example Workflow: Show how one might use Probing (initial check) -> Patching (causal verification) -> SAEs (feature interpretation) -> Causal Abstraction (high-level structure) together to build confidence or identify issues in an NN used for survival prediction or within TL.
*   **Generating Understandable Summaries: Causal Proxy Models:** Explain the concept (building simpler, interpretable models to approximate the NN's causal logic). How it serves as a proxy for understanding. Mention it might use insights from techniques in 4.2 (e.g., important features identified via SAEs/patching). Use case (creating a simple rule set that mimics an NN's treatment effect prediction for specific patient subgroups).
* Connecting Proxy Insights to Actionable Outcomes: How can these proxy findings inform model selection, refinement, trust assessment, or the design of subsequent analyses within the TL framework or broader bio-statistical investigation?




\section{Challenges, Limitations, and Future Directions}\label{mi_challenges}

* Scalability of MI techniques to large bio-statistical NNs.
* Difficulty in interpreting the results of MI itself (e.g., interpreting SAE features, complex circuit diagrams).
* Integrating MI findings effectively into the causal inference workflow (e.g., how does an MI finding update our confidence interval or bias analysis in TL?).
* Need for domain expertise (biology, medicine) to guide and interpret MI results.
* Ethical considerations (e.g., ensuring MI doesn't lead to overconfidence in flawed models).


